Online Advertisements with LLMs: Opportunities and Challenges

This paper explores the potential for leveraging Large Language Models (LLM) in the realm of online advertising systems. We introduce a general framework for LLM advertisement, consisting of modification, bidding, prediction, and auction modules. Different design considerations for each module are presented. These design choices are evaluated and discussed based on essential desiderata required to maintain a sustainable system. Further fundamental questions regarding practicality, efficiency, and implementation challenges are raised for future research. Finally, we exposit how recent approaches on mechanism design for LLM can be framed in our unified perspective.

==> aaai2025/reproduce.tex <==
\section*{Reproducibility Checklist}
Below we give the answers to the reproducibility checklist for this paper. 
\begin{itemize}
    \item Includes a conceptual outline and/or pseudocode description of AI methods introduced: \textcolor{blue}{Yes}
    \item Clearly delineates statements that are opinions, hypothesis, and speculation from objective facts and results:\textcolor{blue}{Yes}
    \item Provides well marked pedagogical references for less-familiare readers to gain background necessary to replicate the paper: \textcolor{blue}{Yes}
    \item Does this paper make theoretical contributions? \textcolor{blue}{No}
    \item All assumptions and restrictions are stated clearly and formally. \textcolor{blue}{NA}
    \item All novel claims are stated formally (e.g., in theorem statements). \textcolor{blue}{NA}
    \item Proofs of all novel claims are included. \textcolor{blue}{NA}
    \item Proof sketches or intuitions are given for complex and/or novel results. \textcolor{blue}{NA}
    \item Appropriate citations to theoretical tools used are given. \textcolor{blue}{NA}
    \item All theoretical claims are demonstrated empirically to hold. \textcolor{blue}{NA}
    \item All experimental code used to eliminate or disprove claims is included. \textcolor{blue}{NA}
    \item Does this paper rely on one or more datasets? \textcolor{blue}{No}
    \item Does this paper include computational experiments? \textcolor{blue}{No}
\end{itemize}

==> abstract.tex <==
% This paper discusses challenges and desiderata to operate an online advertisement system with Large Language Model (LLM).
    % % \slcomment{Although working out the details is part of the point of the paper, it's still too vague to just say ``operating an online ad system with an LLM'' here.}
    % We propose several methodologies to meet those requirements, and verify their validity and discuss advantages and drawbacks of each approach through arguments based on thought experiment.
    % We discuss further technical challenges in implementing and generalizing the system to adapt to practical constraints \sfcomment{We need to add more details to the abstract}
    This paper explores the potential for leveraging Large Language Models (LLM) in the realm of online advertising systems. We delve into essential requirements including privacy, latency, reliability as well as the satisfaction of users and advertisers that such a system must fulfill. We further introduce a general framework for LLM advertisement, consisting of modification, bidding, prediction, and auction modules. Different design considerations for each module are presented.
    Fundamental questions regarding practicality, efficiency, and implementation challenges of these designs are raised for future research.
    Finally, we explore the prospect of LLM-based dynamic creative optimization as a means to significantly enhance the appeal of advertisements to users and discuss its additional challenges.
    % \krcomment{need to rewrite to talk a little bit about personalized ads.}

==> ack.tex <==
\section{Acknowledgements}
The work is partially supported by DARPA QuICC, ONR MURI’2024 award on Algorithms, Learning, and Game Theory, Army-Research Laboratory (ARL) \#W911NF2410052, NSF AF:Small \#2218678, and NSF AF:Small \#2114269, and a grant from an NSF CAREER AWARD 1942230, ONR YIP award N00014-22-1-2271, ARO’s Early Career Program Award 310902-00001, Meta grant 23010098, HR00112090132 (DARPA/RED), HR001119S0026 (DARPA/GARD), Army Grant No. W911NF2120076, NIST 60NANB20D134, the NSF award CCF2212458, an Amazon Research Award and an award from Capital One.
The authors thank S\'{e}bastien Lahaie for valuable discussions.


\section{Conflict of Interest}
The authors find no conflict of interest at the moment.

==> backup.tex <==


\section{Model}
Consider a company owns a large language model (LLM), and runs a LLM-based search engine that displays a result page constructed by the returned output of the LLM based on the user's query.
The company wants to make some revenue through the use of LLM-based search engine.
The most natural way is to borrow the ideas of online advertising system in the traditional search engine.
For example, as most of the traditional search engine makes a tons of profits by incorporating online advertisements into the search engine results page (SERP), the LLM-based search engine can also \emph{intentionally} includes some advertisements within the LLM results page (LRP).
Then, a natural question is how one should add some advertisements within LRP in order to maximize the company's revenue, and how should the advertisers bid on the advertisements?


\paragraph{Structure of LRP}
We can categorize the format of LRP based on the structure of the output.
If we can list the output so that the resulting structure might be similar to traditional SERP, then we call such a structure to be \emph{structured} LRP.
If the user asks LRP to have something different from that, \eg a long text on detailed explanations about some concepts or a combination of figures and texts, then we denote by \emph{nonstructured} LRP.
The methodology for displaying some advertisements may heavily depend on the structure of the output.
For instance, for structured output, there is high probability that one might be able to borrow various approaches in traditional sponsored search auction to have advertisements in the LRP.
For non structured output, however, it is very unclear how one should construct a LRP with advertisement.
We now discuss several ways to generate the final LRP with advertisements. 

\paragraph{Generating response with advertisements}
% \sscomment{Mention simple reduction to SSA for structured output. And then proceed with more challenging nonstructured ones.}
Fundamentally, we consider LLM as a black-box oracle that returns a desired output based on what the user has entered in a prompt.
In particular, as can be seen in some (latest) versions of LLMs, these outputs can be of various formats including figures, LaTeX files, code snippets, etc.
Given a pair of the user's query and the returned output, we consider a scenario in which there exists a collection of advertisers $\cA$ who want to advertise their products by including their products in the returned text in a natural manner.
For example, consider a user who asks to recommend a list of nearby Italian restaurants that is of reasonable prices and walking distances from the user.
Given this specific query, suppose that the company wants to include a specific advertisement of an advertiser, \eg determined by some LLM advertising auction which will be elaborated shortly.
Since LLM is a black-box oracle, it is usually hard for one to make the LLM intentionally changes its output in a desired manner in advance.
Instead, given an \emph{original output}, one can effectively query once more to LLM and ask it to include some advertisements within the new output.
That is, we can consider an existence of a \emph{proxy query engine} who operates as a proxy between the user and LLM to display proper LRP possibly with some advertisements, by asking additional queries to the LLM based on the original query and designated advertisements.
Hence, the fundamental approach to generate a \emph{modified} LRP by incorporating advertisements is for the proxy engine to ask an additional query to the LLM, with some desired advertisements that one wants to append.

\paragraph{Aggregated regeneration}
To begin with on what should be the additional query that proxy engine asks to the LLM to append some advertisements on the output, consider a structured output.
In this case, we have a list of hyperlinks that originally came out of the response of the LRP, and we have a list of advertisements that we want to append.
Suppose we have a list of positions, from $1$ to $k$, that we can append as sponsored advertisements.
Note that in this case, we can exactly borrow the techniques from traditional sponsored advertisements.

For instance, advertisers can bid on some keywords and connect their each of advertisements to several keywords.
Bidding amount can be based on cost per mille (CPM) which charges the advertiser one it is displayed in the LRP, or cost per click (CPC), cost per action (CPA), or so on.
One may differentiate the price based on which position the advertisements are displayed on the LRP, but this is usually incorporated within the click-through-rate (CTR) or conversion-rate (CVR) if the advertisement is charged with respect to CPC or CR.
Based on the bid amounts of advertisements, one can essentially compute the expected revenue of having an assortment of combination of organic list and advertisements, and then optimize over the list of advertisements to display on the LRP.
For instance, for CPC advertisements, one should predict the CTR of the advertisements (for each position) and then multiply it with respect to the bid amount.
Then, given an optimized list of products, one can effectively ask an additional query to the LRP so that it constructs a new output based on the advertisements list, along with the organic LRP it spawns previously.
We denote such an approach by \emph{aggregated regeneration} model.


\paragraph{Direct generation}
On the other hand, in case of nonstructured output, it is not clear how one can bring the traditional techniques into the table.
Here we suggest a new approach to incorporate advertisements into the LRP in this case, which we define as \emph{direct generation} model.
To begin with and clearly present our main insights, we focus on a \emph{text}-based output so that the resulting LRP is entirely a full text.
That said, our approach is not restricted to be text but can be applied for any structure of the output.

Fundamentally, a clear disadvantage of the aggregated regeneration model is that, the bidders should bid on their products without observing the final LRP.
This may not matter that much if the output is going to be very predictable, \eg in case of structured output, but this can be problematic if the output mway vary a lot with respect to the sponsored advertisements.
For example, suppose that the user asks LLM about a detailed technical discussion how computers work.
Then, the LLM may explain the fundamental concept of computation such as logic gates, hardware systems such as RAM, software systems like OS.
Clearly, we can incorporate a tons of advertisements within the LRP, \eg when we explain graphic card we may want to advertise Nvidia on it, and makes some revenue from them.
However, if Nvidia naively bids on some keywords such as graphic cards, without given the context of the LRP context, it may hurt the advertiser's experience.

For instance, if LRP explains that a user who are not interested in computer game or deep learning should not put their much of the budget on graphic card, Nvidia may not want to advertise their product for these contexts since there is low probability that the user will be involved in the advertised products given the contexts.
To handle this case, we consider a \emph{direct generation} model in which the advertisers directly bid on the \emph{final output} of LRP while providing the modified LRP as well.
Basically, the advertisers do not bid in advance on some keywords, but they have a unique API which outputs a bid amount along with a sponsored LRP output.
The input to the API will be a user context, original output of LLM, and the output will be generated LRP and corresponding bid amount.
In words, this is a direct {\bf \em delegated generation} model so that we delegate the role of generating LRP to the advertisers.
However, a disadvantage here is that it is difficult to have multiple advertisements within the final LRP since the bidding mechanism here is restricted to be \emph{advertisers generate and then bid on it}.
That is, it is technically difficult to sell potentially multiple ad slots given a single query.
In addition, this potentially leaks some privacy information of the users to the advertisers, so it is essential to have a user agreement in advance, which will be elaborated more shortly.


For small businesses, however, it is typically impossible to have their own APIs due to technical and budget issues.
In this case, the LLM company can offer them to use an automated own API by the LLM company.
For example, the LLM company may provide a list of {\bf \em autogenerator} that automatically bids while generating a proper sponsored LRP given an advertisement, and the advertiser can decide the type of autogenerator and have a contract on it.
The LLM company may also monetize from the use of autogenerator in this case.\sscomment{this might not be the case, since in the current search engines, they don't charge advertisers from using autobidder, but encourages them to use it as they want to have a full control on the bidding process to optimize more efficiently.}

Finally, given the bid amount and sponsored LRP, a \emph{LLM ad auction} computes expected revenue for each adverisement, and display the most adequate final LRP to the user.
Note that both of the delegated generation model and autobidders can be accommodated within a single advertisement auction after they bid on their own advertisements.

==> bck.tex <==

\section{BCK - Oct 24 21:00}
\subsection{Comparing architectures}
We here compare the architectures we proposed based on the requirements defined in Section~\ref{sec:require}.
\SL{The reader needs to refer back to Section 3 to remember the two options for modification models and bidding models. May be good to reiterate them here.}

\subsubsection{Comparing modification models}
\paragraph{Advertiser modification model}
In the advertiser modification model, LAS should somehow deliver $q,X,C$ to each  $\adv_i$.
If this is the case, this may leak some private information of the user to the bidders, thereby suffering \emph{privacy issues}, which is critical in terms of the user experience.
Partially disclosing the information may help resolve the issue.

In addition, the advertiser modification model has reliability issue since there is a possibility that the advertiser-modified output includes some illegal or spamming contents.
The LAS may devise an additional module to maintain its \emph{robustness} against such kind of adversarial behavior, however, this is still a cost of the LAS to bring them in the system.
This further possibly degrades the user satisfaction since the advertiser-generated output may not be satisfactory for the user compared to what the LLM generates.

Furthermore, this requires additional communication between the LAS and the advertisers, thereby increasing the overall latency.
Overall, advertiser modification model may not be feasible in practice due to several issuses discussed above.

\paragraph{LAS modification model}
On the other hand, LAS modification model does not suffer the privacy, reliability and latency issues.
Furthermore, this model would be more in favor of the user since LAS would basically hope to improve the user experience.
However, one disadvantage is that this may not fully reflect the advertiser's preference on the output modification process, thereby partly decreasing the advertiser's satisfaction.
This issue can be resolved by enabling more flexibility in the architecture, which will be discussed in Section~\ref{sec:extend}.

\subsubsection{Comparing bidding models}
\paragraph{Dynamic bidding model}
The biggest advantage of the dynamic bidding model is that, it would induce higher advertiser's satisfaction rate, thereby attracting more advertisers to participate.
This is because the advertisers have full flexibility in deciding their bids after observing the modified output.
Similar to the advertiser modification model, dynamic bidding model may have privacy issue if LAS discloses some private information to the advertiser.
Moreover, dynamic bidding model may suffer additional latency issue since the entire set of modified output should be delivered to the advertisers.
Note that there is no reliability concern as only the bid amount is communicated.


\paragraph{Static bidding model}
Static bidding model does not suffer any of the privacy, latency, reliability issues.
However, as the advertisers cannot fully customize their bid per each query based on the modified output, this may degrade the advertiser satisfaction. \SL{For readers with a background in auction theory, it's not clear what the allocation functions are here. What do the bids map to exactly?}



% \paragraph{Privacy}
% In the advertiser modification model, LAS should somehow deliver $q,X,C$ to each  $\adv_i$.
% If this is the case, this may leak some private information of the user to the bidders, thereby suffering \emph{privacy issues}, which is critical in terms of the user experience.
% Partially disclosing the information may help resolve the issue.

% \paragraph{Reliability}
% In addition, the advertiser modification model has reliability issue since there is a possibility that the advertiser-modified output includes some illegal or spamming contents.
% The LAS may devise an additional module to maintain its \emph{robustness} against such kind of adversarial behavior, however, this is still a cost of the LAS to bring them in the system.
% % Overall, this model might not be feasible regarding many practical concerns.


% \paragraph{Latency}
% The dynamic bidding model suffers an additional communication burden of delivering $X_i$ to $\adv_i$ for every $i \in [n]$.
% Since the modified output $X_i$ can be a long text possibly with some figures, this may significantly increase the communication cost of LAS, thereby inducing a large \emph{latency} in the overall procedure.
% In addition, since $\adv_i$ cannot directly customize $X_i$ to suit its taste, there might be a chance that the bidder is not very much satisfied with the modified output, thereby possibly decreasing the bid amount.
% However, this approach has privacy gain since LAS does not need to transfer private information of the users to the advertisers.


% \paragraph{User satisfaction}



% \paragraph{Advertisers satisfaction}
% The static bidding model obviously requires far much less communication cost between LAS and advertisers, once after the contract is made, so the overall latency of LAS may be minimal.
% However, this cannot fully reflect the advertiser's preference for each output $X_i$ and corresponding bid $b_i$, possibly decreasing the advertiser's utility.
% In fact, the advertiser who wants to customize their advertising technique might avoid this model.

% \paragraph{LLM provider's revenue}



% \subsection{Extending modification and bidding model}



% \subsection{Robustness}
% In the advertiser modifying model, in order for the advertiser to construct its own outcome, they are required to be provided the original input query.
% This, however, leaks the user's privacy to the advertisers and thus may not be favored by the users.
% Hence, to adapt the delegated generation model, it is important to protect the user's privacy while maintaining the expected quality of the generated outcome by advertisers.

% Also, reliability issue is critical since the output that the advertiser has generated may include a undesired or illegal contents.

\subsection{Extending architectures}\label{sec:extend}
\paragraph{Beyond advertiser and LAS modification}
% Although advertiser modification model enables a~full flexibility for the advertiser to express its preference on the modification, as discussed above, it has critical issues in privacy and robustness as well as the advertiser should somehow develop its own way to modify the output.
% Meanwhile, LAS modification model does not have these issues as LAS directly generates the output, there is a chance that the advertisers are not at all satisfied with the modified output, thereby lowering their bids significantly.
In order to improve the advertiser's satisfaction for the LAS modification module, one approach is to allow the advertiser to submit indirect indicators that represent its preference on what it expects the modified output to be.
More in a detail, once the user asks a query $q$, LAS delivers $q$, the original output $X$, and possibly the context $c$ to the advertiser, and the advertiser returns a string $Y$ that indicates its preference in words.
For example, suppose that $X$ includes a series of laundry machines $a,b,c$.
Having observed what $a,b,c$ is and the original query $q$, the advertiser may return $Y$ as ``advertise product $\ad_i$ after $a$, but before $b$".
After then, LAS may apply their string as a prompt in the LLM to generate the modified output.
This approach allows more flexibility for the advertiser to express its preference on the output.
Note that, however, this still requires additional communication cost compared to the LAS modification model, thereby possibly suffering a latency issue.

\paragraph{Beyond static and dynamic bidding}
Likewise, in the static bidding model, a natural approach to improve the advertiser's satisfaction is to enable a more generic static function as the contract between the advertiser and LLM provider.
For example, the advertiser may specify specific user segments to deliver their advertisements, \eg children under 16, or may screen out some traffics based on geographical information, \eg users far from national parks.
Note that this is often the case in the standard sponsored search auction or display advertisement auction.

% These cases can be modeled as a contract function $f_i:S \times U \times C \mapsto \R_{\ge 0}$ where $U$ denotes the set of user segments and $C$ denotes the set of every possible contexts.
% We denote this model by \emph{contextual} bidding.
% Note that if $f_i(s, u, c) = f_i(s, u', c')$ for every $u, u' \in U$ and $c,c' \in C$, then this corresponds to the keyword bidding.
% Contextual bidding allows the advertisers to make their preference more explicit, thereby possibly increasing their satisfaction.
% \krcomment{i'd simplify this without using function definitions.}

\paragraph{Parallelizing the process and allowing multiple types of advertisers}
Recall that our overall architecture consists of (i) modification, (ii) bidding, (iii) prediction, and (iv) auction modules.
Although each of the process should be serialized in order to handle a single advertiser's process, it is important to observe that the process (i)-(iii) is totally independent between the advertisers.
Hence, one efficient to way to minimize the latency is to process steps (i) to (iii) in an asynchronous manner between the advertisers.
To fit the desired latency requirement, one may consider excluding some advertisers such that the steps (i) to (iii) are not completed within some maximal delay.\SL{It's common to have timeouts in display ads, because bids can come from real-time bidders outside the system, but not as much for search ads as far as I'm aware.}
After collecting all the feasible parameters, LAS can pass the required parameters to step (iv) and run the auction.

One additional advantage of this procedure is that, one can easily adapt to multiple types of advertisers.
In practice, several advertisers may want to dynamically bid or modify the output by themselves, while others with small businesses may not want to take too much of responsibilities.
For instance, consider the following scenario.
\begin{enumerate}
    \item $\adv_1$ wants to modify the output by itself, and dynamically bids on it.
    \item $\adv_2$ does not want to modify the output by itself, but wants to dynamically bid.
    \item $\adv_3$ does not want to modify the output by itself, and wants to bid in a static manner.
\end{enumerate}
If one conceptually separates the steps (i), (ii) and (iii) between the advertisers, we can adapt all of these advertisers by running a separate procedure for each advertiser, and then finally runs the step (iv).


\paragraph{Displaying multiple ads simultaneously}
\SL{We may want to make it clear in the intro that the paper focuses on displaying a single ad, and that multiple ads bring their own challenges discussed briefly at the end.}
\sscomment{Mention it in the intro/model.}
One common feature in the modern sponsored search auction is that, it usually display multiple ads upon a single query, which is mostly to maximize the search engine's revenue.
Given the architecture we proposed, it is not straightforward to allow this feature, so we here discuss several approaches to deal with it.
% We will start from a simplistic scenario, and then gradually complicates it.

First, consider a simple case in which all advertisers use LAS modification and static bidding model.
In this case, one can consider every combination of advertisements as a subset of $[n]$, and then generate modified output with corresponding bid.
Further, if there is an advertiser with dynamic bidding, LAS can simply delegate the bid generating process to that advertiser for every combination that includes this advertiser's ad.


Obviously, these approaches are not computationally feasible if one consider every possible combinations of the subset.
% This is even more problematic if there exists an advertiser with dynamic bidding since the computational burden to communicate the collection of modified outputs can be extremely heavy.
Therefore, the technical challenge lies in how one can optimally decide a subcollection  of the entire power set to balance the trade-off between computational burden with corresponding latency and revenue of the auction.



% First, consider a simple case in which all advertisers use LAS modification and static bidding model.
% Let $\cC$ be a collection of all subsets of the advertisers $[n]$, \ie $\cC = 2^{[n]}$.
% Then, consider an arbitrary subset $C \in \cC$.
% Given the subset $C$, we can generate a modified output $X_C$ such that all the ads $i \in C$ is included in $X_C$.
% For each $X_C$, we can compute its score $s_C$ since all the bids can be computed due to the static bidding model.
% Then, we choose the subset $C^* = \argmax_{C \in \cC} s_C$ that maximizes the score and charges the designated bid as payment for each advertiser.

% In case there exist advertisers who use dynamic bidding, for each $\adv_i$, we can collect the set $\cC_i = \{C \in \cC: i \in C\}$, and deliver the set of modified outputs $\cX_i = \{X_C: C \in \cC_i\}$ to $\adv_i$.
% Once upon receiving $\cX_i$, $\adv_i$ returns a set of bids $\cB_i$ such that $b_C \in \cB_i$ denotes the bid on the modified output $X_C$ for $C \in \cC$.

% For the advertisers with advertiser modification model, it is conceptually not clear to make them modify by considering some of the other advertisers.
% This may fundamentally leak some information of the other advertisers, and the burden for this advertiser will be extremely large as well.
% Therefore, it might be better to exclude this set of advertisers and only consider outputs with single ad for them.





% \paragraph{Market players}
% \sscomment{Suho}


% \paragraph{Measuring output distance}
% As did in the traditional search engine, it is important to measure the quality of the resulting output of the search engine, in order to capture the both rabbits of user retention and instant revenue.
% In particular for the delegated generation model, in order to reliably display the sponsored LRP constructed by the advertisers, there should be a way to measure the quality of the text.
% This controls the trade-off the LLM search engine focusing on long-term user experience to attract the user more into the search engine, and short-term utility of having more advertisements to bring some instant monetary revenue.
% Importantly, whether or not the user regenerates the output will be an important measure for the quality of the output.
% \sscomment{To measure the distance between two documents are major technical challenges.}

% \paragraph{CTR/CVR prediction}
% Note that we can use the output distance as a \emph{feature} of the CTR prediction module.
% Also, unlike from the traditional search engine, the context of output LRP will heavily affect the CTR and CVR of the advertised product.
% For instance, if it was talking about some philosophically negative aspects of online streaming platforms, the CTR of Netflix advertisement will be very low in this case.
% Note also that the regeneration probability accounted above can also be used as a feature of the prediction model as well.

% \paragraph{Privacy}
% In the delegated generation model, in order for the advertiser to construct its own outcome, they are required to be provided the original input query.
% This, however, leaks the user's privacy to the advertisers and thus may not be favored by the users.
% Hence, to adapt the delegated generation model, it is important to protect the user's privacy while maintaining the expected quality of the generated outcome by advertisers.

% \paragraph{Reliability}
% In the delegated generation model, reliability issue is critical since the delegated generated document may include a undesired information.

% \paragraph{Latency}
% If our auctioning process needs outgoing communication via APIs provided by some other companies, this will heavily affect the latency of the entire process.

% \paragraph{Adapt to multiple ad slots}
% In the delegated generation model, since each company generates its own output which only accounts for its advertisement, there is a low probability that the LLM company can fully utilize multiple ad slots which might be available in hindsight.
% \paragraph{Budget smoothing}


% \paragraph{Preprocessing}





\ssdelete{
It is worth noting that the substantial capabilities of generative models empower us to tailor the content of ads itself to individual users,
leveraging their specific contexts to generate more appealing content, which is called as dynamic creative optimization (DCO) or responsive ad in the literature.
This approach holds the potential to significantly boost revenues for both the platform and advertisers.
This concept is detailed in Section~\ref{sec:personalized-ad}..

% \SL{There is a spectrum of possibilities for incorporating ad content into the LLM output. It can range from ads alongside the output (very similar to current search ads), to ads within the output but clearly delineated, to mentions of products within the output as in Table 1. It would be good to acknowledge this and explain if we plan to focus on one type in particular in the paper.}
% \krcomment{what exactly do you mean by ``to ads within the output but clearly delineated"?}
% \krcomment{can we explicitly put names here?}

Then, a natural question is how one can incorporate those advertisements into the generated response.
Unlike the traditional search engine in which the output structure of a single query is regular, \eg a list of hyperlinks to relevant websites, LLM may provide unstructured outputs.
% \SF{this is a bit of strong claims; they can potentially provide lists which can be viewed as a structured output}.
This complicates the process of advertisement in LLMs than that of search engines.
In search engine advertisements, one can simply change the order of search results to include some advertisements.
On the other hand, LLM output can be more general than just a list of items, thus,
one cannot simply include advertisements given the generated output but should construct a way to change the overall output to maintain its quality while including the advertisement.
% \SF{this is not always true; LLMs perhaps can produce a text below that provides links to useful resources; why shouldn't they do that? Without links, only famous brands can be included in advertisements and less known ones would not be recognized}

Another issue is to evaluate the quality of advertisements because advertisers need to bid on modified outputs.
To be more specific, suppose that one has generated a modified output for an advertiser.
If the output is highly unstructured, the quality of advertisement significantly depends on the final manipulated output.
This may further complicate the bidding process since the advertiser may want to allocate a higher bid amount for a modified output with good quality, but not the other way around.
\footnote{For instance, cost-per-click (CPC) or cost-per-mille (CPM) is typical in the modern search and display advertisement systems.
These measures suffice to satisfy advertisers  since the way their ads are displayed is fairly predictable, \eg a predetermined image created by themselves.
If the modified output is largely unstructured in LLM advertisement, however, the advertisers may want to propose tailored bid amount based on the context in which their products are included.
This will be discussed more in details in Section~\ref{sec:discuss}.}
Subsequently, how one should decide which advertisements to include given the vast of advertisers?
%\SL{There is an interesting related area of vector databases which I am just starting to learn about. Not sure whether it's worth bringing up in this paper, but wanted to call it out.}
% \krdelete{
% This includes the question of how each advertiser should bid on their product.
% In particular, suppose that one have generated a modified output for an advertiser.
% Due to the nature of the unstructured output, the quality of advertisement significantly depends on the overall modified output, making it harder to evaluate the quality of the advertisement.
% Correspondingly, this may further complicate the bidding process since the advertiser may want to allocate a higher bid amount for a modified output with a good quality, but not the other way around.}
% \slcomment{In search ads bidders bid per click (CPC), and in display ads it's per impression (CPM). For LLM output there might be a more refined unit of interest/attention/relevance for ads that could be provided by the LLM itself.}
% \sfcomment{rewrite it and make it sharper by start saying: Another issue is evaluating the quality of advertisement ...}
% Furthermore, these complications in the overall process may induce additional challenges in maintaining responsiveness, user privacy, and reliability of the entire system.


% \begin{itemize}
%     \item Modification in which the original output of LLM is modified.
%     \item Bidding that advertisers utilize to bid on the modified outputs.
%     \item Prediction in which the LLM provider computes required information about advertisements.
%     \item Auction in which the advertises compete and the final output is selected.
% \end{itemize}


% \krdelete{These architectures are compared to each other based on their pros and cons, and we discuss further technical challenges to implement the system in a practical manner.}

}



==> conclusion.tex <==
\section{Conclusion}
This paper addresses the opportunities and challenges for leveraging an online advertisement system with LLM.
We first discuss essential requirements which a reasonable LLM advertisement system should satisfy.
To fulfill such desiderata, we introduce several frameworks  and substantiate their validity.
We compare proposed frameworks with their advantages and limitations.
Then we discuss further technical and practical challenges in designing efficient online advertising with LLM.
Finally, as a usecase of independent interest, we present the potential of advanced dynamic creative optimization by using LLM.

% \section{Impact Statement}
% Our paper aims to explore the potential of online advertiseemnt system with LLM and suggests several of its plausible directions in practice. The potential broader impact of our research encompasses several dimensions. Firstly, it advances the practical field of machine learning by initially suggesting several plausible approaches to run online advertisement system for LLM-based search engine. Secondly, our work has implications for the online advertising industry itself, potentially leading to more personalized and targeted advertising campaigns that better align with user interests and preferences.

% Ethically, the deployment of LLM-based advertisement systems prompts considerations regarding user privacy and content reliability. We acknowledge the importance of addressing these ethical concerns and emphasize the need for responsible implementation practices and mechanisms.

% Furthermore, the societal consequences of our work include shaping the digital landscape and influencing user experiences on online platforms. As online advertising plays a significant role in shaping consumer behavior and influencing purchasing decisions, our work may impact the dynamics of online commerce, search engine and corresponding consumer engagement.

% \section{Impact Statement}
% \sscomment{To be done}

==> discussion.tex <==
\section{Challenges}\label{sec:discuss}
Recall that our overall framework consists of four modules: modification, bidding, prediction, and auction module.
For each module, we discuss several characteristics, technical challenges, and corresponding research questions in implementing the proposed architectures in practice, evaluating their overall practicality with respect to the criteria defined in Section~\ref{sec:require}.
We provide further discussions in Appendix~\ref{apd:further-discuss}.

\definecolor{challenge-fg}{rgb}{0.9, 0.2, 0.2}
\definecolor{challenge-bg}{rgb}{0.98, 0.5, 0.44}

\subsection{Modification module}
% \begin{tcolorbox}[colback=challenge-bg,colframe=challenge-fg]
% \begin{center}
%   Advertiser modification model that guarantees no privacy-issues, reliability, user satisfaction, and low-latency.
%   \end{center}
% \end{tcolorbox}
 {\color{red}Challenges:} {\bf Advertiser modification model that guarantees no privacy-issues, reliability, user satisfaction, and low-latency.}
In the advertiser modification model, LLMA should somehow deliver $q,X,C$ to each  $\adv_i$.
This may leak some private information of the user to the bidders, thereby suffering \emph{privacy issues}, which is critical for user experience.
It should be addressed how LLMA can partially or indirectly disclose the information to prevent user privacy while guaranteeing high quality output from the advertiser modification module.
\ssedit{Partially disclosing the information based on its level of privacy concern, using encryption, or the notion of differential privacy might be useful in this regard.}
% Partially disclosing the information may help resolve the issue, but 
% {\bf Research question: implementing advertiser modification module with less privacy issue}


In addition, the advertiser modification model has reliability issue since there is a possibility that the advertiser-modified output includes some illegal or spamming contents.
The LLMA may devise an additional module to maintain its \emph{robustness} against such kind of adversarial behavior, however, this is still a cost of the LLMA to bring them in the system.
This further possibly degrades the user satisfaction since the advertiser-generated output may not be satisfactory for the user compared to what the LLM generates.

Furthermore, this requires additional communication between the LLMA and the advertisers, thereby increasing the overall latency.
\ssedit{As such, developing an efficient protocol and algorithm to implement is necessary to operate a reasonable online ad system.}
Advertiser modification model faces many concerns as discussed, thereby requiring innovative methodologies from several perspectives to resolve all these issues.
% Overall, advertiser modification model may not be feasible in practice due to several issues discussed above.
% {\bf Research question: guaranteeing reliable, user-satisfying, low-latency output from advertiser module.}

\vspace{0.3cm}
\noindent {\color{red}Challenges:} {\bf Effectively reflecting advertiser preference on the output for LLMA modification model.}
On the other hand, LLMA modification model does not suffer the same amount of privacy, reliability and latency issues mentioned above.
Furthermore, this model would be more in favor of the user since LLMA would aim to improve the user experience.
However, one disadvantage is that this may not fully reflect the advertiser's preference on the output modification process, thereby partly decreasing the advertiser's satisfaction.
Thus, it should be explored how one can effectively reflect advertisers' preference on the modified output to better capture the output that advertisers would have preferred.

% This issue can be resolved by enabling more flexibility in the architecture, which will be discussed in what follows.
% {\bf Research question: well-reflecting advertiser's preference on the output.}
\vspace{0.3cm}
\noindent {\color{blue}Prospect:} {\bf Balancing the trade-off between LLMA/advertiser modification models.}
% Although advertiser modification model enables a~full flexibility for the advertiser to express its preference on the modification, as discussed above, it has critical issues in privacy and robustness as well as the advertiser should somehow develop its own way to modify the output.
% Meanwhile, LLMA modification model does not have these issues as LLMA directly generates the output, there is a chance that the advertisers are not at all satisfied with the modified output, thereby lowering their bids significantly.
In order to improve the advertiser's satisfaction for the LLMA modification model, one approach is to allow the advertiser to submit indirect indicators that represent its preference on what it expects the modified output to be.
More in a detail, once the user asks a query $q$, LLMA delivers $q$, the original output $X$,
and possibly the context $c$ to the advertiser, and the advertiser returns a string $Y$ that indicates its preference in words.
% For example, suppose that $X$ includes a series of laundry machines $a,b,c$.
% Having observed what $a,b,c$ is and the original query $q$, the advertiser may return $Y$ as ``advertise product $\ad_i$ after $a$, but before $b$".
After then, LLMA may apply $Y$ as a prompt in the LLM to generate the modified output.
This approach allows more flexibility for the advertiser to express its preference on the output.
Note that, however, this still requires additional communication cost compared to the LLMA modification, which possibly increases latency.
Another way to better capture advertisers' preference on valuations without further communication is to ask advertisers to write a list of documents to give it as samples to the LLM as a prompt engineering.
% {\bf Research question: a framework that balances the trade-off given by LLMA modification, and advertiser modification models.}

\subsection{Bidding module}\label{sec:discuss-bidding}

% \paragraph{Comparing bidding models}
 {\color{red}Challenges:} {\bf Implementing dynamic bidding model without privacy and latency issue.}
The biggest advantage of the dynamic bidding model is that, it would induce higher advertiser's satisfaction rate, which may be attractive for some advertisers who have technical capability to dynamically send bid with respect to the proposed output.
This is because the advertisers have full flexibility in deciding their bids after observing the modified output.
Similar to the advertiser modification model, dynamic bidding model may have privacy issue if LLMA discloses some private information to the advertiser.
Moreover, dynamic bidding model may suffer additional latency issue since the entire set of modified output should be delivered to the advertisers.
Note that there is no reliability concern as only the bid amount is communicated.\footnote{
Note that static bidding model does not suffer any of the privacy, latency, reliability issues.
However, as the advertisers cannot fully customize their bid per each query based on the modified output, this may degrade the advertiser satisfaction. }
Overall, the research in this direction should carefully address how practical the dynamic bidding model is, and which protocol and algorithm could implement such model without violating privacy and latency issue.\footnote{Further, one may also investigate how the ad market would comprise of, when there is a possibility that the advertisers hire a proxy agent to write bid on behalf of them, and how the proxy agent (or advertisers themselves) can optimize bids in such scenario.}


% {\bf Research question: implementing dynamic bidding without privacy/latency issue.}
% {\bf Research question: Advertiser needs a way to evaluate the quality of the output. How can this be made practical?}

% \sscomment{research question?}
% \slcomment{For readers with a background in auction theory, it's not clear what the allocation functions are here. What do the bids map to exactly?}
% \sscomment{it may be discussed in Auction module part at Section 4. Could you see if more elaboration would be needed?}


\vspace{0.3cm}
\noindent {\color{blue}Prospect:} {\bf Balancing the trade-off between static/dynamic bidding models.}
% \paragraph{Beyond static and dynamic bidding}
% \sscomment{change title}
In the static bidding model, a natural approach to improve the advertiser's satisfaction is to enable a more generic static function as the contract between the advertiser and LLM provider.
% For example, in a simplistic approach, the advertiser may specify certain user segments to deliver their advertisements, \eg children under 16, or may screen out some traffics based on geographical information, \eg users far from national parks.
Specifically, LLMA can propose the bidding contract as a function that maps an indirect measure of the modified output to a nonnegative real number representing the bid, \ie the advertiser's valuation.
% between the quality of the modified output to a non-negative real number. 
For instance, LLMA and an advertiser agrees on a inverse proportional contract based on the similarity distance $d$ between the original output $X$ and the modified output $X_i$.
For example, if $X_i$ is examined to be very different form $X$, then $d(X,X_i)$ will be large, and then the advertiser's valuation, \ie bid, on $X_i$ is small since it is believed that the incorporation of ad too much changed the content of the output, thereby hurting user experience and capturing less user attention.
% For instance, the bidding function on the committed contract can be a linear function that is proportional to the distance measure between the modified output and the original output, \eg charge $\$5 \cdot d$ if the similarity distance is $d$.
Note that in this case, the advertiser may need to partly understand how LLMA estimates the distance measure and how it's defined.
More generally, LLMA might construct a more refined way to measure the user's interest, attention, relevance for the modified output from the perspective of $\adv_i$, and let the advertisers commit to either of the contract based on its taste.
These are crucial aspects to explore to run LLMA in practice.

\subsection{Prediction module}
{\color{red}Challenge:} {\bf Efficient and precise implementation of prediction module.}
% To recap, the input to both the prediction modules is the original output $X$, query $q$, context $c$, and the modified outputs $(X_i)_{i \in [n]}$.
The process of estimating CTR will be analogous to that in the modern online advertisement system.
We can train a prediction system to predict $\ctr_i \in [0,1]$ given the input $X_i, q, c$ for each $i \in [n]$ based on the feedback data from the user.\footnote{For instance, as is typical in the modern online advertisement system, one may use factorization machine based online algorithm after extracting some features from user, context, and the queries. More detailed discussion can be found in \cite{mcmahan2013ad}.}
As discussed in Section~\ref{sec:pred}, since $X_i$ will be very sparsely appear if the entire document is considered as an embedding, we may extract some useful features from each $q, X_i$ and $c$, and learn the mapping from features to the true value.
Whether the user regenerates the response, clicks the ad, or exits the LLM, can be used as feedback data to improve the prediction module.

% Feedback data will be the direct action of the user indicating whether they click the ad or not.\sscomment{awkward sentence}
% This prediction system can be trained in an online manner to update the estimate in (almost) real time, which will increase the accuracy of the prediction.
% \sscomment{move the footnote to the main body?}
% {\bf Research question: }
\vspace{0.3cm}
\noindent {\color{red}Challenge:} {\bf Relevance/similarity distance measure to estimate user satisfaction.}
To estimate SR, one may first consider an explicit approach given an assumption that the \emph{original output is optimal}.
If we assume that the original output is optimal, then essentially a \emph{distance} between the original output $X$ and the modified output $X_i$ will be a good measure to predict the SR since if $X_i = X$, then the user will be the most satisfied.
In this context, given the original $X$, one may use the marginal probability $\Pr{X | q}$ as an indicator for SR.
For example, one can define \emph{output distance} by $d(X, X_i) := ||\Pr{X | q}, \Pr{X_i|q}||$ for some proper norm.
Note that the probability for an output to be obtained can be computed via standard method in the literature~\citep{vaswani2017attention}, by computing the probability distribution in a token-by-token manner.
Further, one can consider more general distance function $d$, \eg the semantic similarity of two documents/phrases \citep{mikolov2013efficient, cer2018universal, conneau2019unsupervised}.
Essentially, a concrete research question in this context is to identify a good measure to capture the user's satisfaction in advance when ads are incorporated in the output.
% {\bf Research question:  }
% Due to the nature of the LLM's output generating process, given a sequence of string token $t_1, t_2, \ldots, t_k$, we can compute the conditional probability $\Pr{t_{k+1} | t_k, t_{k-1}, \ldots, t_1}$ which denotes the probability that the token $t_{k+1}$ is generated given the history.
% In particular, this procedure is possible since given a sequence of tokens, we can obtain the distribution over the next tokens.
% For each $X_i$, denoting the entire string $S(X_i)$ as a sequence of tokens $(t_1^i, t_2^i, \ldots, t_{l_i}^i)$, the marginal probability $\Pr{s(X_i)}$ can be computed using the tower rule, \ie $\Pr{s(X_i)} = \prod_{j=1}^{l_i}\Pr{t_{i+1} | t_i, t_{i-1},\ldots, t_1,q}$ where we abuse $\Pr{t_1 | t_0, q}$ to denote $\Pr{t_1 | q}$.
% Then, a distance between $\Pr{s(X_i)}$ and $\Pr{s(X)}$ given some metric can be used as the indicator for the user's satisfaction rate.
% We denote this \emph{output distance} by $d(X, X_i) := d(\Pr{s(X)}, \Pr{s(X_i)})$ where $d$ denotes some valid metric.
% Note that this does not involve any learning process, but just require a series of computation to obtain the probability.

\vspace{0.3cm}
\noindent {\color{blue}Prospect:} {\bf Incorporating distance measure and online learning.}
As discussed above, one may consider combining the approaches of distance measure and online learning from user feedback for SR prediction.
% Alternatively, we can \emph{learn} SR via feedback data from the user.
To online learn SR estimates from user feedback, a useful indicator of whether the user is satisfied with the output is whether the user \emph{re-generates} the output given the same (or similar) query.
Hence, one may aim to learn a function which outputs the $\sr$, given the query $q$, modified output $X'$, and context $c$.
This approach does not assume that the original output $X$ is indeed optimal, thereby allowing the possibility that the user may be satisfied with a modified output $X_i$ even though its distance from $X$ is measured to be far.
Note that one should implement an independent training system to operate this learning process, leading to additional burden for LLMA.
To incorporate advantages of these two approaches, one can consider an online learning model where the distance is also integrated as one of the features to predict it, \ie $d(X,X_i)$ is used as a feature of the SR prediction system.
In case $d(X,X_i)$ indeed has some positive correlations with the true user satisfaction rate, this would increase the accuracy of the prediction.
Essentially, an effective way to capture the both advantages of online learning and distance measure should be studied thoroughly.



\subsection{Auction module}\label{sec:discuss-auction}
% \paragraph{Adjusted}
{\color{red}Challenge:} {\bf Incorporating multiple ads in a single output.}
% \paragraph{Multiple ads at once}
Recall that in our auction module, the modified output is fully determined based on the allocation function so that if it is allocated to $\adv_i$, then the modified output $X_i$ will be displayed to the user.
One approach to generalize this framework is, to let the final output to be displayed the one that does not necessarily belong to $\{X_i\}_{i \in [n]}$, but rather a new output $X'$ that somehow interpolates $\{X_i\}_{i \in [n]}$.\footnote{We discuss further comparison to the token auction model by~\cite{duetting2023mechanism} in Appendix~\ref{sec:discuss-comparison}.}
Let us denote the new output $X'$ by \emph{balanced output}, \eg see Table 2 in~\cite{duetting2023mechanism}.
By doing so, it might be possible to deliver multiple advertisements in a fair manner,\footnote{Another way to display multiple ads at once will is discussed in Appendix~\ref{sec:challenge-apx} under our original framework.} thereby allowing LLMA to bring more revenue by charging multiple advertisers at once.
One subtle issue is that, since each advertiser bids $b_i$ on delivering $X_i$, they may not want to write the same bid for the balanced output $X'$, thus it may degrade the advertiser's experience on participating in the LLMA.\footnote{In the static bidding model, as discussed in Section~\ref{sec:discuss-bidding}, this might be handled by committing to a contract based on measures that represents the advertiser's preferences more in a refined manner.
In the dynamic bidding model, one approach would be to append an additional step of asking for bids for the final output again to the advertisers.}
In summary, incorporating multiple ads in a single response is technically challenging, which would require both theoretical and practical studies to validate reasonable approaches.

% \sscomment{Shorten it}
% In the static bidding model, as discussed in Section~\ref{sec:discuss-bidding}, this can be handled by committing to a contract based on measures that represents the advertiser's preferences more in a refined manner.
% In the dynamic bidding model, of course, this may simply be handled by incorporating additional steps of querying the bid for the final output again.

% {\bf Research question: reasonable way to adjust advertiser's bid for the multi allocation mechanism for both dynamic and static bidding models?}




\section{Dynamic Creative Optimization via LLM}
\label{sec:personalized-ad}
\input{personalized-ad}

Now, we discuss about the possibility of advanced dynamic creative optimization by using LLM.
\emph{Dynamic creative optimization} (DCO)
\footnote{This is often called as dynamic product ads (DPA), but DPA typically refers to the process of selecting which item to advertise from a given catalog of an advertiser, whereas DCO denotes the process of modifying the ad itself.},
in the traditional search and display ad markets, refers to the technique of dynamically adjusting the combination of ad assets and constructing an advertisement that best fits the customer's preference.
It can markedly enhance the quality and relevance of the ad to the user by tailoring the contents of ad in a personalized manner.
Many online advertisement platforms adopt DCO-based ads, which is often called as \emph{responsive ad}~\citep{GoogleAdSearch,GoogleAdDisplay}.
\footnote{As traditional DCO is restricted to dynamically construct the complete image file of ad, we here restrict our attention to the image-based ads as well. However, it is apparent that LLM based DCO would work beyond image-based ads.} 
% \krcomment{Fantastic footnote!}}

In the canonical DCO framework, a static ad consists of a single image file that can only be displayed in a specific set of ad channels, whereas dynamically optimized ad consists of a single ad template and multiple options for each asset that fills in the ad template.
This is typically done by the advertiser registering multiple options for each asset given an ad template, and then the system picks the optimal combination.
% \footnote{Note that this is different from picking and delivering the most relevant ad given a pool of ads, but about tailoring the ad itself to satisfy the user.}
This procedure aims at increasing the CTR and SR, which would eventually improve the welfare efficiency of the online ad ecosystem~\citep{mcmahan2013ad} as well as the revenue of the ad platform.


% It's important to recognize that tailoring advertisements to individual preferences can enhance their quality, making them more appealing to users.
% Consequently, the user's satisfaction rate tend to rise, accompanied by an increase in the click-through rate when exposed to personalized advertisements.
% This positive correlation leads to higher revenue for both LLM provider and advertisers, aligning with the goals of the effective advertisement.
% This brings more revenue for LLM provider as well as advertisers and improves user experience, thereby increasing the welfare efficiency of the online ad ecosystem~\cite{mcmahan2013ad}.

Unlike from the traditional DCO techniques, the arise of LLM, especially those support the output with image such as ChatGPT 4, enables more involved process of dynamic creation of ads, as well as replaces the role of traditional DCO in online ad platforms.
For example, given a user query and context, the platform may send a query to LLM to customize the image of ad to attract the user by capturing user preference.
We provide representative examples in Figure~\ref{fig:personalized-ad} where two scenarios of personalizing ads is depicted.
Note that the use of LLM-based DCO is not restricted to LLMA, but can be broadly applied to SA and display ad.

\vspace{0.3cm}
\noindent {\color{red}Challenge:} {\bf Refining each module.}
% \paragraph{Incorporating responsive ad}
To integrate responsive ads, a more advanced modification module is imperative.
This module should not only enable the alteration of the original response to include ads but also incorporate them in a manner that takes into account user preferences.
This entails utilizing user contexts, \eg gender/location/the current device used for the query, in the ad generation process.
To be more specific, the modification module should incorporate user context in the process of modifying the original response.
This makes ads more appealing to the user by considering their preferences.
Leveraging language models, we can prompt them to factor in various elements related to user context during the generation of modified outputs.
As illustrated in Figure~\ref{fig:personalized-ad}, information about users' context can be utilized to create more captivating advertisements for them.

Further, the prediction module may interact with the modification module to commit to the modified output that mostly increases user's experience, \ie CTR and SR.
Even for SA, the prediction module may need to be made more sophisticated to predict the CTR and SR of the responsive ads.
This is in stark contrast to the standard DCO since it may not significantly change the ad image overall, but only slightly changes the part of it by replacing some ad assets.
Correspondingly, the advertiser may value the generated ad differently, \ie write different bid, with respect to the quality of the ad generated by LLM-based DCO.
Overall, a vast amount of studies should be done to clearly investigate a plausible framework for LLMA, even for SA, to adapt the LLM-based DCO.

\vspace{0.3cm}
\noindent {\color{red}Challenge:} {\bf Meeting system requirements.}
Obviously, running LLM-based DCO should not entail the failure of the system requirements discussed in Section~\ref{sec:require}.
For instance, in terms of latency, we observed that generating an image with the GPT4 takes almost about $10$s for Figure~\ref{fig:personalized-ad}.
Given that the online advertising typically requires the ad latency up to $100$ms, the required latency is almost $100$ times the conventional threshold.
Thus, the fundamental research challenge is to enable a fast production of an ad image to meet the conventional latency requirement in the online advertising system.
Further, it will be technically interesting to balance the tradeoff between the ad's quality and latency which governs the advertiser and user utility, respectively.

% Finally, we remark that these involved process demand additional computational resources, potentially impacting latency when incorporating responsive ads.
% Online advertisement typically requires the overall latency of real time bidding process to be within $100$ms, however, we experience several second of delay to modify the image output presented in Figure~\ref{fig:personalized-ad}. 
% Thus, it is technically interesting to balance the tradeoff between the ad's quality and latency, \eg naively by using cache, and also it might be possible to pass along part of such cost to the advertisers via monetary charge.

Interestingly, as acute readers may have noticed, Figure~\ref{fig:personalized-ad} includes some technical issues in the images themselves.
For example, the first image in the car ads generate a word that is not easily understandable.
Indeed, LLM-based DCO may induce the reliability issue due to the hallucinating nature of LLM \citep{Ji_2023, guerreiro2023hallucinations, bubeck2023sparks}.
Thus, LLM-based DCO should ensure that it does not generate a hallucinated ad that may hurt the advertiser satisfaction.
A simple approach might be to require LLM to minimally revise the reference images, requesting the advertisers to submit several images for reference.

% \krcomment{Keivan: write something about hallucination, LLM alignment, etc in temrs of research challenges. Cite some papers. ALso discuss Travel ad and point out some issues.
% }


% {\color{red}Challenge:} {\bf Reliability and LLM alignment.}
% }

% {\bf Research question: Challenges in modification, prediction, bidding.}



% \sscomment{Add one more para discussing issues in the figure. And then discuss research challenge.}


% \sscomment{todo: polish this para}
% \ssdelete{
% Beyond the modification module, both the prediction and bidding modules require adjustments, given the integration of user context in new ads.
% Bidders now face the task of not only assessing the quality of the modified output in terms of advertisements but also determining its appeal to the user.
% Moreover, as new modified outputs have the potential to be more enticing for users, CTR and SR may witness an increase.
% Consequently, the prediction modules also need to take user context into account and evaluate whether personalized ads can enhance CTR and SR or not.
% }

% In our framework, the feasibility of responsive ads is evident, albeit with the trade-off of increased complexity in the system.
% It's essential to acknowledge that 


\vspace{0.3cm}
\noindent {\color{red}Challenge:} {\bf Cost sharing model.}
Unlike from the traditional DCO technique that simply determines the efficient combination of ad assets, LLM-based responsive ad can do much beyond by creating truly new content.
On the other hand, such process necessarily entails increased use of computational resource, especially since more queries to LLM will be required to customize the ads.
We here discuss several plausible cost sharing models that LLMA might adopt.

The simplest one will be to charge the advertisers whenever the contents are dynamically modified.
For example, the advertiser and LLMA commit to a mutual contract on how much the advertiser pay the LLMA for each responsive ad, and LLMA charges the advertiser whenever it responsively modifies the ad contents.
As the advertiser might hope to use responsive ad only if the user context is sufficiently relevant to its ads, the contract might specify when the advertiser's ads will be responsively changed.
Also, LLMA may provide several options for advertiser to determine how frequently and largely it should responsively modify the ads.

This model would work well for those charged by cost-per-impression, however, advertisers with cost-per-click or cost-per-conversion may not willingly commit to the contract since they desire to pay the platform only if the actual click or conversion happen, even though the platform indeed responsively modified its ads for every impression.
LLMA might give several options to the advertisers under which event they will be charged to pay for responsive ad.
Ads with cost-per-click model may still want to pay for responsive ads per impression or per click.
For the latter, LLMA may offer a larger amount of commission per click by predicting the average CTR of the ads.

LLMA must also decide whether or not to account the increased amount of payment for each advertiser as the increment of the actual bid or just regard it as a separate commission.
For the former case, the advertisers who are willing to charge more for the responsive ad commission fee will take advantage of getting higher chance of delivering their ads, compared to those who do not use responsive ad option.
By doing so, the auction module can select the ad that truly maximize the total revenue expected from delivering a single advertisement, thereby increasing the platform's revenue.

% {\bf Research question: How to reasonably charge advertiser}

% These concerns can be all resolved if LLMA decides to incorporate the increased amount of payment for each advertiser as the increment of the actual bid.
% More precisely, for cost-per-click ad with per-click commission for responsive ad, LLMA can essentially estimate the CTR of the ad and estimate the total revenue of delivering the responsive ad.
% Moreover, LLMA can charge the advertiser 

% or just regard it as a separate commission.



% For (ii), 


% Importantly, LLMA must decide whether or not to account the increased amount of payment for each 
% % We need to talk about privacy as well.

% Importantly, 

% One another consideration is to determine how much frequently LLMA will personalize the ad contents.





% {\bf Research question: DCO with respect to the latency issue.}

% \sscomment{Cost sharing model? We change per impression. But advertiser may want to pay per click. Charge part of costs or not?}

% \sscomment{Contract between ad / platform. We may need to avoid always personalization.}

% \sscomment{Are we going to add this as an actual "bid", or are we keeping them separate?}


% We note that our framework also supports personalized ads.

% In case the advertisers use LLMA modification model,
% one further improvement that LLMA can incorporate is to personalize the advertisement messages or figures based on what the advertise provides as ad creatives.
% The gains from this procedure might be more significant if the modified output contains advertisement as a figure inside the output.
% For example, suppose that an advertiser who wants to advertise its brand new desktop products with several models.
% Consider a user who asks LLM about how a desktop computer operates overall.
% LLM may provide an illustrative figure to describe how a computer operates in general.
% Depending on the user's context, \eg gender/location/the current device used for the query, it is possible to personalize the advertisement by incorporating the suitable model that the user may prefer the most.
% This procedure can not only increase the revenue of the advertiser and LLMA, but also improve the user experience.



% First, consider a simple case in which all advertisers use LLMA modification and static bidding model.
% Let $\cC$ be a collection of all subsets of the advertisers $[n]$, \ie $\cC = 2^{[n]}$.
% Then, consider an arbitrary subset $C \in \cC$.
% Given the subset $C$, we can generate a modified output $X_C$ such that all the ads $i \in C$ is included in $X_C$.
% For each $X_C$, we can compute its score $s_C$ since all the bids can be computed due to the static bidding model.
% Then, we choose the subset $C^* = \argmax_{C \in \cC} s_C$ that maximizes the score and charges the designated bid as payment for each advertiser.

% In case there exist advertisers who use dynamic bidding, for each $\adv_i$, we can collect the set $\cC_i = \{C \in \cC: i \in C\}$, and deliver the set of modified outputs $\cX_i = \{X_C: C \in \cC_i\}$ to $\adv_i$.
% Once upon receiving $\cX_i$, $\adv_i$ returns a set of bids $\cB_i$ such that $b_C \in \cB_i$ denotes the bid on the modified output $X_C$ for $C \in \cC$.

% For the advertisers with advertiser modification model, it is conceptually not clear to make them modify by considering some of the other advertisers.
% This may fundamentally leak some information of the other advertisers, and the burden for this advertiser will be extremely large as well.
% Therefore, it might be better to exclude this set of advertisers and only consider outputs with single ad for them.





% \paragraph{Market players}
% \sscomment{Suho}


% \paragraph{Measuring output distance}
% As did in the traditional search engine, it is important to measure the quality of the resulting output of the search engine, in order to capture the both rabbits of user retention and instant revenue.
% In particular for the delegated generation model, in order to reliably display the sponsored LRP constructed by the advertisers, there should be a way to measure the quality of the text.
% This controls the trade-off the LLM search engine focusing on long-term user experience to attract the user more into the search engine, and short-term utility of having more advertisements to bring some instant monetary revenue.
% Importantly, whether or not the user regenerates the output will be an important measure for the quality of the output.
% \sscomment{To measure the distance between two documents are major technical challenges.}

% \paragraph{CTR/CVR prediction}
% Note that we can use the output distance as a \emph{feature} of the CTR prediction module.
% Also, unlike from the traditional search engine, the context of output LRP will heavily affect the CTR and CVR of the advertised product.
% For instance, if it was talking about some philosophically negative aspects of online streaming platforms, the CTR of Netflix advertisement will be very low in this case.
% Note also that the regeneration probability accounted above can also be used as a feature of the prediction model as well.

% \paragraph{Privacy}
% In the delegated generation model, in order for the advertiser to construct its own outcome, they are required to be provided the original input query.
% This, however, leaks the user's privacy to the advertisers and thus may not be favored by the users.
% Hence, to adapt the delegated generation model, it is important to protect the user's privacy while maintaining the expected quality of the generated outcome by advertisers.

% \paragraph{Reliability}
% In the delegated generation model, reliability issue is critical since the delegated generated document may include a undesired information.

% \paragraph{Latency}
% If our auctioning process needs outgoing communication via APIs provided by some other companies, this will heavily affect the latency of the entire process.

% \paragraph{Adapt to multiple ad slots}
% In the delegated generation model, since each company generates its own output which only accounts for its advertisement, there is a low probability that the LLM company can fully utilize multiple ad slots which might be available in hindsight.
% \paragraph{Budget smoothing}


% \paragraph{Preprocessing}






% \subsection{Designing score function}
% \sscomment{this will be a common issue in search auction. Should we discuss it?}
% How should we design the objective function to maximize the company's revenue in the long run?
% If we do not care about the user retention, \ie satisfaction rate, then one can simply use $\Obj(\sr, \ctr, \bid) = \ctr \times \bid$ to maximize the myopic revenue.
% Since this may hurt the user experience a lot, a simple remedy might be to include a indicator function with a static threshold, \eg $\Obj(\sr, \ctr, \bid) = \ctr \times \bid \times \Ind{\sr \ge \tau}$.
% In this way, one may prevent the modified output hurting the user experience too much, while trying to maximize the advertisement revenue.
% Alternatively, one may separate the user satisfaction rate $\sr$ and the company's revenue $\ctr \times \bid$, and then select a proper Pareto optimal point among $(\sr_i, \ctr_i \times \bid_i)$ for $i \in [n]$.

% Recall the fundamental reason that one should consider the user's experience is to increase the user retention and to compete with other platforms, search engines, etc.
% In a similar context, to deliver high-quality advertisements with more revenue, it is also important to attract more advertisers.
% This implies that we should also account for the advertiser's utility to compete with other online ad platforms., which is often captured by \emph{efficiency} in the modern sponsored search auction.




==> extended-related.tex <==
\section{Related works}
 % \krcomment{i'll add some stuff later.}
\krcomment{we can have extended review of literature in Appendix. I think this section should be done in a single column.}
\paragraph{Large Language Models}
The intersection of artificial intelligence, natural language processing, and conversational agents has witnessed significant advancements in recent years.
The advent of the Transformer architecture, introduced in \cite{vaswani2017attention}, laid the foundation for large language models.
Transformers, with their self-attention mechanism, revolutionized the way models capture contextual information, enabling superior performance on NLP tasks.
By scaling up those architectures, OpenAI's GPT-3 \citep{brown2020language} and Google's BERT \citep{devlin2019bert} are obtained, revolutionizing the field of chatbots, enabling more natural and contextually relevant interactions. 
Those models showed remarkable performance on the natural language generation task leading to the development of chatbots and conversational AI systems.
These chatbots engage in context-aware, human-like conversations, offering valuable solutions in customer service, healthcare, and educational domains \cite{abd2020effectiveness, nicolescu2022human}.

\paragraph{Online Advertisement}
Online advertising, particularly within the context of sponsored search auctions, has evolved in recent years,
with notable contributions from prior research.
Sponsored search auctions have been a subject of extensive investigation, emphasizing the optimization of bidding strategies and keyword relevance.
Notably, \cite{edelman2007internet} provided valuable insights into the economics of sponsored search auctions,
shedding light on the intricate dynamics of keyword auctions.
We refer to the book by \cite{roughgarden2010algorithmic} for more detailed discussion.
\slcomment{This citation is a book chapter, not an entire book.}

\paragraph{Chatbot advertisement}
\sscomment{Skip this or move to the appendix}
With emergence of chat-bot in various websites,  several companies started to run a chat-bot advertisement, which is often referred to as sponsored message.
In the chat-bot advertisement, the companies send some private messages on the chat-bot conversation to advertise some products.
This is very different from operating an~online advertisement system over LLM, since chat-bot advertisement simply sends some messages, but our model captures the scenario in which the user asks a query and then LLM provides a output including some advertisements.
Notably, Microsoft Bing started to operate an online advertisement with Bing chat-bot (\eg see articles ~\cite{Adweek, Techcrunch, Microsoft}).
Indeed, once the user inputs a query in the chat-bot, the output often includes advertisements with explicit flags that indicates this is an advertisement.

\paragraph{Mechanism design with LLM agents}
Interestingly, \cite{duetting2023mechanism} recently proposes a mechanism design problem when the bidders are LLM agents.
More specifically, the bidders bid on desired distributions of the \emph{next token}, given the history of the tokens.
They denote this problem by \emph{token auction}, and provide theoretical foundations of what a reasonable mechanism should look like.
Indeed, their model can be considered as a version of our advertiser modification and dynamic bidding model.
Notably, they require the advertisers to provide their desired distribution and corresponding bidding for every token, which may require significant communication burden to run the mechanism in practice.
In stark contrast, the advertisers in our model only bid once for the modified output, thereby inducing less communication cost.
Nevertheless, we discuss how one can adapt their model into our framework and interpolate between two models, thereby taking the advantages of both models.

\paragraph{Dynamic creative optimization}
\ssedit{
Dynamic Creative Optimization (DCO) is an online advertising strategy that involves dynamically tailoring the content of an ad based on user behavior, demographics, and user context~\cite{baardman2021dynamic}. 
Instead of displaying a static, one-size-fits-all ad, DCO allows advertisers to create and serve personalized and relevant ad content to different audience segments.
By doing so the platform can improve the likelihood of user engagement, click throughs, and conversions.
DCO typically involves the use of technology and algorithms to automate the process of selecting and assembling ad elements, such as images, copy, and calls-to-action, in real-time. This customization is done based on user data, collected either in real-time or from previous interactions. 
Unlike DCO has been typically used only in display advertising not search advertising~\cite{choi2020online} since the tailored ad creatives, \eg personalized hyperlinks to websites, would not have much impact for structured output of standard search engines.
Due to the unstructured nature of LLM advertisement, the use of techniques similar to dynamic creative optimization would be highly likely to be present in future.
Our paper suggests the use of LLM, more generally generative AI, to personalize the advertisement itself  to improve the relevance and quality of the advertisement.
}



\sscomment{We may mention the following in the appendix (borrowed from other paper, need to revise in our own words):::::
In addition to the help of LLM or generative AI for the dynamic creative optimization, it can be used to help the advertisers and marketers to construct their static ads.
For example, many platforms such as Copy.ai, Jasper.ai, Peppertype.ai help to create text-based marketing content for marketers.
Further, DALL-E2 can be used in generating realistic visuals and artworks based on text-to-image prompts. 
More importantly, digital advertising giants such as Meta have made tools available to
their clients. For instance, in May 2023, Meta announced a generative AI Sandbox that offered advertisers access to three tools to help advertisers in various ways, \eg create variations of ad given the input ad, constructs background through text prompts, or change the ad format to fit in various platforms such as social media or short video platform.
}

% To the extent of our knowledge, however, this is the first paper to discuss technical challenges and feasible architectures in leveraging online advertisement system with LLM.


% Recently, several tech companies started to run Chatbot advertisements.


% \begin{enumerate}
%     \item Chatbot advertising effectiveness: When does the message get through?. This paper is about Facebook sending "sponsored message" to the user, which is very different from what we are doing. This is basically referred to as Chatbot Marketing
% \end{enumerate}
% Several reference links that consider similar questions here, mostly by Microsoft Bing.
% \begin{enumerate}
%     \item \href{https://www.adweek.com/media/microsoft-details-how-advertising-works-on-bings-ai-driven-chat-based-search/}{article 1}
%     \item \href{https://about.ads.microsoft.com/en-us/blog/post/may-2023/a-new-solution-to-monetize-ai-powered-chat-experiences}{article 2}
%     \item \href{https://techcrunch.com/2023/03/29/that-was-fast-microsoft-slips-ads-into-ai-powered-bing-chat/}{article 3}
%     \item \href{https://www.thedrum.com/news/2023/03/30/gpt-4-powered-bing-chat-introduces-ads-and-experts-believe-it-s-natural-fit}{article 4}
% \end{enumerate}



==> intro.tex <==
\section{Introduction}

% \kredit{need to rewrite to talk a little bit about personalized ads.}
In the vast landscape of online search engines, the role of advertisements has become pivotal, shaping the digital experience for users globally.
The enormity of the market, with trillions of dollars at play, underscores the economic significance of advertising, \eg the market size of search advertisement as of $2020$ was valued at USD $164.12$ billion~\citep{AdScale}.

Online advertising not only brings revenue to platform companies, but also plays a crucial role in subsidizing the free access to information and service to every individual.
% In a world where people increasingly expect free access to information and services, advertisements play a crucial role in subsidizing these offerings. 
The democratization of education, information, and other resources is made possible through ad-driven models, enabling individuals to not only consume content for free but also contribute to the digital ecosystem. 
Additionally, the symbiotic relationship between advertisements and content creation creates a feedback loop, fostering economic growth.
As a side note, even the subscription-based streaming platforms like Netflix are starting ad-supported plans~\citep{Netflix}.
% Several online platforms often offer a subscription model for people to disable the advertisement in using their services, however, the advertisement market is becoming increasingly dominant, \eg Netflix recently started an ad-supported plan~\cite{Netflix}. 

On the other hand, recently, large language models (LLMs)~\citep{brown2020language,anil2023palm,thoppilan2022lamda} have gained widespread adoption among users,
serving various functions including question answering, content generation, translation, code completion,
and more \citep{nijkamp2022codegen, fried2022incoder, wang2021gpt, liu2023visual}.
The proliferation of AI-driven assistant language models, such as ChatGPT,
has contributed to a growing trend wherein individuals increasingly use such models to address their inquiries,
occasionally replacing traditional search engines as their primary information-seeking tool.
According to~\cite{PCMag}, even for now, $35\%$ of casual users say they find LLMs to be more helpful in finding information than search engine.
It is obvious that such a trend will be accelerating in the near future as well.
The substantial usage volumes stemming from diverse users would induce companies offering these tools, which we call \textit{LLM providers},
to contemplate revenue generation through advertising~\citep{Adweek, Techcrunch, Microsoft}.
Consequently, an interesting and fundamental question arises: 

\definecolor{mycolor}{rgb}{0.9, 0.90, 0.9}
\begin{tcolorbox}[colback=mycolor,colframe=gray!75!black]
\begin{center}
  How can \textbf{LLM providers} make revenue by running an online \textbf{advertisement} on it?
  \end{center}
\end{tcolorbox}


The concept of online advertising has been extensively studied within the realm of search engines, where auctions are conducted among advertisements from advertisers when a user inputs a query.
This paper focuses on the prospect of transposing this online advertising model and auction framework to the context of large language models.
We further discuss technical challenges and potential framework to run online advertisement system in LLM, thereby calling academic and industrial researchers to the area of importance.

\input{prompt-intro}

\paragraph{Search advertising}
To better explain fundamental differences between the standard search advertising (SA)\footnote{Its mechanism design problem is often called as sponsored search auction (SSA).} and the LLM advertising (LLMA), we briefly introduce how the standard SA works~\citep{lahaie2007sponsored} in what follows.
(1) {\em Bidding}: in the SA, the owner of each ad $i$ writes bid $b_i \in \R_{\ge 0}$ on targeting \emph{keyword} for $i \in [n]$, which can possibly a set of keywords.
(2) {\em Output generation}:  the platform first decides \emph{how many slots} to allocate for ads in the search engine results page (SERP), say $k$.
(3) {\em Prediction}: given $k$ slots in SERP, the platform then predicts the click-through-rate (CTR) $\alpha_{ij}$  when ad $i$ is allocated in slot $j$.
(4) {\em Auction}: then it optimizes 
\begin{align}
    \max_{x \in [0,1]^{n \times k}}\sum_{i=1}^n \sum_{j=1}^k \alpha_{ij}b_i x_{ij},\label{eq:alloc-sa}
\end{align}
where $x = (x_{ij})_{i \in [n], j \in [k]}$ is the (possibly randomized) allocation vector such that $x_{ij} = 1$ if ad $i$ is allocated in slot $j$ given the constraint $\sum_{i=1}^n x_{ij} \le 1$ for every $j \in [k], i \in [n]$, and charges each ad with respect to the committed payment rule.

Overall, whenever a user arrives in the platform and searches a keyword, the set of ads related to the keyword are getting involved in the mechanism.
Specifically, the platform collects corresponding bids, decides the number of slots $k$, predicts CTR, and the auction runs.

% \begin{enumerate}
%     \item Bidding: In the SSA, the owner of each ad $i$ writes bid $b_i \in \R_{\ge 0}$ on targeting \emph{keyword} for $i \in [n]$, which can possibly a set of keywords.
%     \item User interaction: Whenever a user arrives and searches a keyword, the advertisers who specified that keyword automatically participates in an auction.
%     \item Output generation: The platform first decides \emph{how many slots} to allocate for ads in the search engine results page (SERP), say $k$.
%     \item Prediction: Given $k$ slots in SERP, the platform then predicts the click-through-rate (CTR) $\alpha_{ij}$  when ad $i$ is allocated in slot $j$.
%     \item Auction: the mechanism optimizes $\sum_{i=1}^n \sum_{j=1}^k \alpha_{ij}b_i x_{ij}$, where $x_{ij} = 1$ if ad $i$ is allocated in slot $j$, given the constraint $\sum_{i=1}^n x_{ij} \le 1$ for every $j \in [k]$, and charges each ad with respect to precommitted payment rule.
% \end{enumerate}



% If the platform runs a generalized second price auction, which is fairly common in practice~\cite{milgrom2004putting}, it sorts the ads by $\alpha_1 b_1 \ge \alpha_2 b_2 \ge \ldots \ge \alpha_n b_n $, and select top $k$ ads.
% Each selected ad is charged the lowest bid necessary to retain its position, \ie $\ell$-th highest selected ad is charged $\alpha_{\ell + 1}b_{\ell+1}/ \alpha_{\ell}$ for $\ell \in [k]$.


\paragraph{Motivating example}
How would the LLMA be fundamentally different from the SA?
We start with illustrative scenarios where a user asks a technical question about computers (Figure~\ref{fig:intro}).
Without advertisement, LLM would typically generate a response to address the user's query.
% To incorporate advertisements in the generated response and induce user attention, there is a spectrum of possibilities for including ad content: (a)  putting the ads outside the response but in the user interface, (b) incorporate the ads within the generated output directly. \krcomment{later we refer to structured and unstructured output (e.g. Figure~1 caption), but they are not defined here -- is footnote enough?}
% \sscomment{I thought the contents in footnote a bit hurt the flow here, and it might be fine to just let it be in footnote. Do you think we should move it to the main body?}
(a) can be deemed as display ads, and would be relatively easy to handle given the vast amount of techniques in display ads.
However, (b) is more similar to search ad or native ad.\footnote{Typically, search and native ads capture user attention much better than display ads, \eg viewed $\sim 50\%$ more than display ads~\citep{NativeSearch}.}
We will focus on the approach (b), which will entail fundamental challenges that have \emph{not arisen} in the traditional SA.
\footnote{Also, in case the ads are included within the generated output, there are several possibilities such that the ads may simply replace one of the element in case they are written as a list of elements (\eg Figure~\ref{fig:intro2}, denoted by \emph{structured} output), or the ads itself is incorporated within the original text/figure without hurting/changing the context of the original output (\eg Figure~\ref{fig:intro}, denoted by \emph{unstructured} output). We focus on the case of unstructured output, as this would be broadly applicable in various scenarios, and the structured output may be able to handled with the standard SA framework.}
% (a) ads alongside the output, (b) explicitly putting advertisements in the output like display ads, and (c) including advertisements within the generated output.


\paragraph{SA versus LLMA}
Recall the process of bidding, output generation, prediction, and auction in the SA mentioned before, and imagine implementing those modules for LLMA.

For the bidding module, how could the advertisers \emph{write bid}?
What would they actually \emph{bid for}?
This is not straightforward to answer, since the user query in LLM cannot be simply specified as a keyword.
Further, given that the marketing impact will be significantly dependent to how the LLM incorporate the ad in the output, it is not even clear what is the advertiser's \emph{value} for being included in the ad. 
% \krcomment{I'd merge this and next paragraph (remove the empty line)}
In fact, the advertiser's value would be dependent to the generated output, then again, how could the advertiser reflect their \emph{willingness-to-pay} with respect to the output, which might not be accessible in advance?
Even further, how can we generate output that smoothly incorporates the ad without hurting the user experience while satisfying the advertiser?

For prediction module, most SA run an online learning algorithm to update the ad's feature vector with respect to the user context~\citep{mcmahan2013ad}.
This was possible because the ad images, hyperlinks, and more generally how they appear in the SERP remain the same across many user interactions.
LLM, however, would incorporate ad in a very different manner for each query, \eg see Figure~\ref{fig:personalized-ad}, then how can the LLMA \emph{learn the CTR} fundamentally?
Also, since the ads are merged into the generated output, it significantly affects the user experience, then how can we guarantee the user satisfaction and measure them?

Finally, which kind of auction format should LLMA run? How can LLMA adapt for advertising multiple ads in a single output?
What would be a reasonable analogue of the autobidding system prevalent in the modern online ad system?

All these questions are not straightforward to answer, yet, have not been formally discussed in any literature to the extent of our knowledge.




% \sscomment{Mention more about difference}
% How to construct the output/ how bidders bid/ how to predict CTR/ 

% We will focus on the case where the ads are incorporated in the unstructured output of the LLM, since the other cases could be handled using techniques from modern online search/display advertisement system.
% Moreover, this kind of advertisement can be more interesting for both users and advertisers due to the huge capabilities of language models in generating high-quality responses while promoting products and services from advertisers.\footnote{Indeed, it's worth noting that Microsoft Bing has been running such types of advertisements in its AI chatbot~\cite{Microsoft}.}

% Then, a natural question is how the system can incorporate advertisements into the generated output to satisfy both the advertisers and the user.
% Further, it is not trivial how the advertisers should communicate with the system to bid on each modified output.


\paragraph{Our contribution}
In this paper, we introduce a vast amount of research questions to operate LLMA in practice.
We first discuss several desiderata to run LLMA and propose a seemingly plausible framework to meet the requirements.
Similar to SA, our framework consists of four modules, though the implementation of each module will be very different from SA:
(i) \emph{modification} in which the original output of LLM is modified;
(ii) \emph{bidding} that advertisers utilize to bid on the modified outputs;
(iii) \emph{prediction} in which LLMA computes required information about advertisements; and
(iv) \emph{auction} in which the advertises compete and the final output is selected.
We discuss different designs and technical challenges of each of those modules, along with further research challenges to implement the system in a practical manner.
\footnote{We first focus on presenting a single advertisement in the LLM output,
however, generalization of the proposed framework to incorporate multiple ads at once is discussed in Section~\ref{sec:discuss-auction}.}
We correspondingly raise several research questions on different design choices for each module.
Although we believe that our framework may be grounded as an initial stepping stone for future research, our primary prupose is to discuss research questions that should be addressed for the practical operation of LLM advertisement.


Finally, as an independent interest, in Section~\ref{sec:personalized-ad},
% as an LLM's (more generally generative model's) use case of independent interest
we discuss how LLM (more generally generative model) can empower the online advertisement system to tailor the content of ads itself to individual users,
leveraging their specific contexts to generate more appealing content, which is called as \emph{dynamic creative optimization} (DCO) or \emph{responsive ad} in the literature.
The incorporation of DCO into the SA, especially for LLMA, would bring further challenges in each module and we propose corresponding research questions therein.
% boost the modern \emph{dynamic creative optimization} technique to improve both the user and advertiser experience.
% It is worth noting that the substantial capabilities of generative models empower us to tailor the content of ads itself to individual users,
% leveraging their specific contexts to generate more appealing content, which is called as dynamic creative optimization (DCO) or responsive ad in the literature.
% This approach holds the potential to significantly boost revenues for both the platform and advertisers.
% This concept is detailed in Section~\ref{sec:personalized-ad}.
% \krcomment{ensure that intro is done within first two pages. we can shirnk some paragraphs and remove redundant phrases.}






==> meeting.tex <==
\section{Meeting Dec 6th}
\begin{itemize}
    \item See Retrieval-Augmented Generation for Knowledge-Intensive NLP Tasks. $p(z | x)$ is affected by the bid
    \item Generate Image and inserting ad?
    \item Want to generate different image. (Focus on image). Auction mechanism? Bidders bid on image?
    \item Or, given the ad creative, change the ad creative based on the query so that the click probability increases. (it is actually used in search auction)
\end{itemize}

\section{Meeting Nov 2nd}
\begin{enumerate}
    \item Experiments
    \begin{enumerate}
        \item What kind of Distance function, and their correlation to the SR - Amazon Mturk (Probably we can use each distance function as a feature and build some models to predict SR.)
        \item Test if advertiser would like the modified output?
        \item The other idea is ...
    \end{enumerate}
    
\end{enumerate}

==> model.tex <==
\section{Framework for LLMA}
\input{teaser}
% \SF{this is our proposed pipeline for LLMA;}
In this section, we present overall framework for LLMA.
We introduce several feasible types of architectures for LLMA, each of which has its own advantages and disadvantages that will be discussed together.
Mainly, we focus on a scenario in which a user provides a query $q$ to the LLM, and the original output by LLM is given by $X$.
Further, a context $c$ captures a variety of features that are relevant to the advertisement recommendation, \eg history of the previous queries, user segment, region, and date.
Although the number of advertisers (bidders) varies from time to time, at the moment the user inputs the query $q$, we suppose that there are $n$ advertisers indexed by $V = \{\adv_1,\adv_2, \ldots, \adv_n\}$.
For simplicity, we assume that each advertiser $\adv_i$ is equipped with a single advertisement (ad) he/she wants to post.
We denote $\adv_i$'s ad by $\ad_i$ for $i \in [n]$, and let $D = \{\ad_1,\ldots, \ad_n\}$.

Overall, we divide the LLMA as follows based on their functionalities\footnote{These functionalities may be distributed to multiple market players such as supply side platform, display side platform, or ad exchange, as does in the current online ad eco-system.}
into $4$ modules: (i) output modification, (ii) bidding, (iii) prediction, and (iv) auction. 
% \begin{itemize}
% 	\item Output modification module
%     \item Bidding module
% 	\item Prediction module
% 	\item Auction module
% \end{itemize}
This overall framework is illustrated in Figure~\ref{fig:teaser}. In short, 
\begin{enumerate}
    \item The user asks a query $q$ to the system along with a context $c$;
    \item The LLMA generates the original output $X$;
    \item The modification module generates specific output $X_i$ for each of the advertisers;
    \item The bidding module generates corresponding bid $b_i$.
    At the same time, the prediction module predicts the quality of the output $X_i$ by measuring the user satisfaction rate $\sr_i$ and click-through-rate $\ctr_i$;
    \item Finally, the auction module runs auction to determine the final output and corresponding payment amount to charge the advertiser.
\end{enumerate}

% In short, the user asks a query $q$ to the system along with a context $c$, and the LLMA first generates the original output $X$.
% Then, the modification module generates specific output $X_i$ for each of the advertisers, and the bidding module generates corresponding bid $b_i$.
% At the same time, the prediction module predicts the quality of the output $X_i$ by measuring the user satisfaction rate $\sr_i$ and click-through-rate $\ctr_i$, which will be elaborated later.
% Finally, the auction module runs auction to determine the final output and corresponding payment amount to charge the advertiser.
% \sscomment{Add enumeration}
% Also, note that we do not restrict the final output to be exactly belonging to one of $X_i$, but can be totally different one based on the advertisers' bids $b_i$ and corresponding output $X_i$.
% \sscomment{fix this clearly}
For the rest of the section, we will explain each module and its responsibility/functionality in a sequential manner.

\subsection{Modification module}
The modification module takes responsibility for generating modified output based on corresponding ads.
This module takes the pair of $(q,X,c)$ and a set of advertisements $D$ as the input, and returns $(X_i)_{i \in [n]}$ where $X_i$ denotes the modified output for $\ad_i$.

Overall, we consider two approaches based on who generates the modified outputs.
\footnote{
For either cases, one can generate the modified output by giving an additional query to the LLM as presented in Figure~\ref{fig:intro}.
}
\begin{enumerate}
    \item In the \emph{advertiser modification} model, the role of generating the modified output is delegated to each advertiser, and collect the modified outputs from them.
    \item In the \emph{LLMA modification} model, LLMA directly generates the modified output.
\end{enumerate}

% In either model, there would be several ways to modify the output.
% For example, one can do a prompt engineering by manually writing static sentences that are parameterized by the ads and append them to the original query.
% Alternatively, one may consider each advertisement as a document in a context of retrieval-augmented generation by~\cite{lewis2020retrieval}, and generates the final output by conditioning on the documents.

\paragraph{Comparison to SA}
Note that the standard SA does not have modification module explicitly as it is trivial to incorporate ads in each slot.
Thus, we emphasize that is the challenge that uniquely appears in LLMA.

% \sscomment{At the end of each subsection, add a para discusses difference vs SSA.}



\subsection{Bidding module}
The bidding module generates bid based on the modified outputs.
The input to the bidding module is the query $q$, context $c$, and modified outputs $(X_i)_{i \in [n]}$, and the output will be a bid $(b_i)_{i \in [n]}$, where $b_i$ is the bid for $ad_i$.
Similar to the generation model, we consider two models for the bidding module.
\begin{enumerate}
    \item 
    In the \emph{dynamic bidding} model,  we deliver relevant information, \eg query $q$, context $c$, the original output $X$,\footnote{To protect the user's privacy, one may consider delivering an encrypted context $\hat{c}$ or the one that excludes private information.} along with the modified output $X_i$ to the bidder for each query, and then the bidder returns the corresponding bid.
    \item In the \emph{static bidding model}, each bid is determined by some keywords based on some pre-committed contract, without any additional communication with the advertiser.
\end{enumerate}

The static bidding model would be able to be operated by extracting some keywords from the user query and run the bidding based on the keywords while asking advertisers to bid on each keyword, similar to the SA.
In Section~\ref{sec:discuss}, we discuss several extensions of these bidding models, thereby allowing more flexibility for advertisers to customize their advertisement strategy by bidding.


Dynamic bidding model may be of interest to the advertisers who have their own measures to estimate the quality of the modified output and thus want to customize their bid in a way that might not be captured by the static bidding.
For example, in extreme, suppose that LLMA may only consider click-through-rate of the modified output and does not care about the user satisfaction rate or how much the inserted advertisement relates to the context of the output.
In this case, the advertiser may want to customize their bid by measuring the quality of the output by itself, since he may be afraid of the system inserting its ads in an awkward manner.

\paragraph{Comparison to SA}
Note that in SA, since the context of user query in search engine is more explicit, and can typically abstracted as several keywords, advertisers can safely bid on each keyword.
In LLMA, however, it might be difficult to extract proper keywords from the query as the query itself tends to be much longer than the traditional SA due to the flexibility of LLM.
Further, the generated output significantly affects the marketing impact of the ads in LLMA, whereas it is typically assumed (and validated) to be independent from other ads / contents shown within SERP in the standard SA.
Finally, the dynamic bidding model further exhibits unique challenges of requiring advertisers to dynamically adjust the bid with respect to the output.

% \sscomment{Why exactly the bidders change bid? If just bid on click? What if bidding on sth else? Discuss: Various measure that might not be captured by the platform, then advertiser may want to customize. Platform may have different measure}

% If LLMA runs the dynamic bidding model, advertisers should somehow implement the bidding API which outputs a proper bid given the relevant parameters.
% This, however, will be difficult for some small businesses.
% In this case, they may 

% In the static bidding model, we further consider \emph{keyword-based} bidding and \emph{contextual} bidding.

% \subsection{Ad Generation and Bidding Module}
% \sscomment{Separate modules}
% This module takes responsibility of generating modified output based on corresponding ads, and bidding with respect to the modified output.
% Given the inputs described above, we propose several models for ad generation and bidding module.
% We propose two dimensions to categorize the module based on (i) who generates modified outputs, and (ii) whether the bidders bid dynamically or statically.
% For the first category, we introduce \emph{Advertiser generation model} and \emph{LLMA generation model}.
% In the advertiser generation model, we delegate the role of generating the advertisement to each advertiser along with corresponding bid, and then LAA runs.
% Meanwhile in the LLMA generation model, LLMA generates the advertisement for sake of each bidder
% For the second category, we consider \emph{dynamic bidding model} in which we provide relevant features along with the modified output to the bidder for every query and then the bidder dynamically bids on the output, and \emph{static bidding model} where each bid is determined by some keywords or features based on some pre-committed contract.
% We consider all possible combinations based on two category but bidder generation with static bidding model, since if bidder directly generates the output then it is natural for bidder to attach the corresponding bid upon it.

% \paragraph{Advertiser generation and dynamic bidding}
% In this model, given query $q$, original output $X$, and context $c$ each $adv_i$ generates $X_i$ along with the corresponding bid $b_i$.
% Then, LLMA collects the pair of modified output and bid $(X_i, b_i)_{i \in [n]}$ along with some additional information from prediction module which will be described shortly, it delivers all the required parameters to the LAA.
% After then, LAA runs and the final winner and corresponding payment function will be determined.

% To this end, importantly, LLMA somehow delivers such information $q,X,C$ to each bidder $b_i$.
% If this is the case, however, this may leak some private information of the user to the bidders, thereby suffering a \emph{privacy issue}, which is critical in terms of the user retention.
% Therefore, this model might not be feasible in practice.
% % Furthermore, since it might not be easy for the advertisers to implement output generation system, this may spawn a \emph{third-party player} in the online ad eco-system who operates as a proxy between the advertisers and LLMA to generate modified output for sake of the advertiser.
% % These will be discussed more in details in Section TBD.


% \paragraph{LLMA generation and dynamic bidding}
% In this model, given $q, X, c$, the ad generation module generates the modified output $X_i$ for sake of the advertiser $adv_i$ for $i \in [n]$.
% Since there is a possibility that the advertiser does not like the modified output a lot, the most precise way for proposing a proper bid for the modified output is to deliver $X_i$ to $adv_i$, and collect the returned bids $b_i$.
% Then, similar to the model above, LAA runs with the required collected parameters and determine the final output of the auction.


% \paragraph{LLMA generation and static bidding}
% Similar to the previous model, auctioneer generates each of $X_i$, but also determines $b_i$ without additional communication with the advertisers.
% This can be made possible by both the auctioneer and advertiser committing to a contract in advance, which explicitly states the bidding method based on the relevant parameters.
% In its simplest form, advertiser $i$ may specify a set of keywords $K_i$ and corresponding bid $b_{K_i}$, and then if $X_i$ includes one of the keywords $K_i$ then bidding module will bid $b_{K_i}$ for $X_i$, and then LAA runs.
% We denote this by \emph{keyword bidding}.
% Advertiser $i$ may specify multiple sets of keywords $(K_{i,j})_{j \in [m_i]}$ and corresponding $b_{K_{i,j}}$ for each $j \in [m_i]$.
% Note that these examples can be generalized by determining a function $f_i:S \mapsto \R_{\ge 0}$ for a set of every possible string (keyword) $S$, \ie a mapping from a string (keyword) to nonnegative real numbers denoting the bid amount.


\subsection{Prediction Module}\label{sec:pred}
Prediction module is responsible for computing user's satisfaction-rate (SR) and click-through-rate (CTR).
User's SR indicates how much the user is satisfied with the given output.
This SR affects the final decision making process of LLMA since if there is a chance that the user is very disappointed with the modified output, then it should reconsider displaying that output as it may hurt the user experience a lot.
On the other hand, CTR indicates the probability that the user clicks the ad link included within the modified output.
This is also critical in determining the auction winner since this directly affects the revenue of the LLMA.
More precisely, if an advertiser's bidding method is cost-per-click (CPC), then CTR proportionally affects the advertisement revenue as the expected revenue of transferring its ad can be computed as CPC times the CTR.
% That said, CTR may not play an important role for advertisers with bidding type cost-per-mille (CPM), since the revenue is fixed once their ads are displayed.
Overall, both of SR and CTR can be defined as a function of original output $X$, modified output $X'$, query $q$, and context $c$, which returns a real value in $[0,1]$.
Detailed methodologies for estimating/learning these functions will be discussed in Section~\ref{sec:discuss}.

\paragraph{Comparison to SA}
Different from the traditional SA whose output is static (as ad image/hyperlinks), LLMA constructs the output in a highly dynamic manner. 
This makes the prediction module more difficult to learn the CTR.
Moreover, in LLMA, the prediction of user satisfaction is much more directly affected by the incorporation of the ads in the output.
This is in stark contrast with SA, whose user experience is usually affected only by the number of ad slots in SERP.




\subsection{Auction module}
Computed all the required parameters above, we finally run the auction module to determine who wins the auction and how much the advertiser will be charged.
The input to the auction module is the tuples of $(\bid_i, \sr_i, \ctr_i)_{i \in [n]}$ which denotes bid amount, satisfaction rate, and click-through-rate, respectively.
Output of the auction module is an allocation $a \in \{0,1\}^n$ and a payment $p \in \R_{\ge 0}$.
Precisely, auction module determines the auction format which consists of the allocation function and the payment function, where the allocation function decides which advertisement to deliver and the payment function computes how much the advertisers pay LLMA.\footnote{In its current form, this does not allow the possibility of adjusting the final output in order to balance between multiple advertiser's preferred output.  Our framework, however, does not preclude possibility for such extension, which we will elaborate more in Appendix~\ref{apd:further-discuss}.}
% determines the mechanism $\textsc{Auc}: \R^3 \mapsto \{0,1\}^n \times \R^n$, where $\{0,1\}^n$ denotes the allocation function and $\R^n$ in the codomain denotes the payment function.
% For example, if the output is determined to be allocated to $\adv_i$ given the allocation function, LLMA will display $X_i$ to the user while charging the advertiser based on the payment function.


Importantly, the main goal of LLMA is to maximize its revenue in a long term manner.
To this end, this should balance a trade-off between short-term revenue and the user retention.
Therefore, the objective can be modeled as a function from bid amount, CTR, and SR to a nonnegative real number that indicates a score of a modified output, \ie selecting $i^* = \argmax_{i \in [n]} \Obj(\sr_i,\ctr_i, \bid_i)$.
We do not discuss how to choose the objective function here, given the vast literature on the sponsored search auction.
% \krcomment{this paragraph can be shortened by providing less mathematical details. I don't think notations like $\mathbb{R}$ are necessary.}
% \sscomment{Removed notations}
After designing the score function, one should determine an auction format.
Also, given the long line of literature on auction design, one can pick the most preferred mechanism, \eg first-price auction (FPA) or second-price auction (SPA).



\paragraph{Comparison to SA}
The main difference to the SA is, similar to what is discussed in the previous subsection, the user satisfaction is much more important measure to account for.
For example, the allocation function in SA represented by~\eqref{eq:alloc-sa} is social welfare which only accounts for platform and advertisers' utility.
In LLMA, however, one might also need to consider user's utility as a function of predicted SR, which would change the allocation function of the mechanism and the payment correspondingly.

% To briefly provide some examples, most modern online advertisement platforms use either of first-price auction (FPA) or second-price auction (SPA).
% SPA has a theoretical advantage of being incentive-compatible, thereby inducing a simple strategy of truthful bidding for the advertisers.
% Not being incentive-compatible, however, many big-tech companies run FPA for their online advertisement auctions.
% For instance, Google changes their auction format from SPA to FPA recently.
% The main reason behind such decision was that it significantly simplifies the overall advertisement process, which happened to become very complicated as lots of market players and modules came in.
% In addition, as many advertisers delegate the role of bidding process to the online ad company by using \emph{autobidder}, where the advertiser simply puts a budget threshold and then the company optimizes the bidding process for sake of the advertiser, FPA has its own advantage of simplifying this optimization procedure since the payment can be directly computed only by its bid.



==> preliminaries.tex <==
\section{Preliminaries}
\sscomment{Making Notations Consistent: LLM provider, LLM Advertisement System (LAS) (Use this one mostly), Ad modification, Bid generation, Prediction module, LLM Advertisement Auction (LAA)}
Large language models (LLMs) have gained widespread adoption among users, serving diverse functions including question answering, content generation, translation, and more. The proliferation of AI-driven assistant language models, such as ChatGPT, has contributed to a growing trend wherein individuals increasingly turn to such models to address their inquiries, occasionally supplanting traditional search engines as their primary information-seeking tool.


The substantial usage volumes stemming from diverse users have prompted companies offering these tools to contemplate revenue generation through advertising. Consequently, an interesting question arises: how can companies providing these services effectively generate revenue through advertising mechanisms?

The concept of advertising has been extensively investigated within the realm of search engines, where auctions are conducted among  advertisers when a user inputs a query. We focus on the prospect of transposing this advertising model and auction framework to the context of language models, exploring the potential challenges and disparities in this context. In this paper, our primary focus revolves around evaluating various architectural approaches for this purpose and recommending the one with the least inherent limitations and challenges.
\sscomment{move three to intro}


We start by an illustrative scenario where a user asks a technical question about laptops \sscomment{provide some figure example.}. Without advertisement, an AI assistant tool would typically generate a response to address the user's query. However, within the content of the generated response, there exists an opportunity for the chatbot to strategically incorporate advertisements for laptop manufacturers, such as Apple, Microsoft, ASUS, and others.


In the context of user-initiated searches for laptop-related queries, manufacturers of laptops may express interest in inserting relevant links leading to their respective websites. This engagement aims to facilitate users' exploration of their product offerings.
In light of these considerations,
several important questions arise, requiring careful examination:

\begin{itemize}
    \item \textbf{Mechanism for modifying LLM output for advertising}: how to change LLM output to incorporate advertisement?
    \item \textbf{Efficieny of content manipulation}: Given the imperative of delivering timely responses to user queries, the process of manipulating output should be fast.
    \item \textbf{Responsibility of output modification}:
    Should it be the role of the company providing the AI-bot, or should advertisers themselves undertake the task of tailoring the content to advertise their products and services? This aspect warrants a comprehensive evaluation.
\end{itemize}


\paragraph{Mechanism for modifying LLM output for advertisement}
We note that advertising in the output of a LLM usually corresponds to adding keywords, inserting links to advertisers' websites, or generating some texts to promote companies' products.
However, 
maintaining the quality of the revised output is paramount; the chat-bot must continue to furnish the user with output of commendable quality. Consequently, any alterations introduced into the output must not compromise its informativeness, accuracy, or overall utility.
Furthermore, as users expect real time performance from these chat-bots, the process of modifying output should be fast. Users anticipate swift responses, necessitating a streamlined and efficient mechanism for incorporating modifications without undue delay.


Indeed, the task of modifying the original output generated by a language model is a complex and multifaceted endeavor. This task encompasses a range of strategies, spanning from relatively straightforward approaches like keyword insertion to more nuanced techniques involving paraphrasing the original content while seamlessly integrating keywords or links.
\sscomment{good sentence}


Moreover, contemporary AI-chatbots are endowed with the capability to accept prompts that instruct them to adapt or manipulate input text. For instance, users can prompt a language model like ChatGPT to make specific alterations to a given text, such as incorporating particular keywords or external hyperlinks.

\paragraph{Responsibility of output modification}
\sscomment{Somehow overlaps with the subsequent section}
When considering the process of obtaining new output from the original output generated by a Large Language Model (LLM), two fundamental approaches emerge:
\begin{itemize}
    \item 
    \textbf{Advertiser-Centric Modification:}
    \sscomment{Advertiser modification}
    In this approach, companies take the initiative to modify the LLM's original output by injecting their preferred context or promotional content into the response. Essentially, advertisers directly customize the output to align it with their specific messaging, keywords, or links.

    \item
    \textbf{Chat-bot Provider Facilitated Modification:}
    \sscomment{LAS modification}
    In contrast, the responsibility for modifying the output rests with the chat-bot provider, which operates the LLM. Companies interested in advertising submit requests to the chat-bot provider, specifying the desired changes they wish to see in the response. The chat-bot provider then incorporates these modifications into the original output.
\end{itemize}

In the context where advertisers are tasked with modifying the original output generated by a Large Language Model (LLM), specifically when a user inputs a prompt and the LLM generates the initial response, advertisers interested in promoting their products or services for that particular user query are required to customize the original output to align it with their promotional objectives. This process typically involves providing advertisers with access to user information, the user's query, and the original LLM-generated output. However, this approach comes with a series of notable challenges:

\begin{itemize}
    \item There might be users' privacy concerns when user's information, and query is given to advertisers.
    
    \item how does the advertiser should change the output in a way that the final output remains high-quality? In this case, we should assume that the advertiser needs having access to language models capable of generating high-quality outputs. Furthermore, generated output should be evaluated by original model, thus, requires advertisers to obtain some knowledge over the original model to be able to generate output that is accepted by chat-bot.
    
    \item as the final output is generated by advertisers, original chat-bot should ensure that this output is safe, high-quality, and responds to user's query. As a result, another phase of evaluating proposed outputs should be run. Furthermore, chat-bot evaluation method shouldn't be vulnerable, as any kind of vulnerability may lead to scenario where the adversary can inject harmful, junk, or low-quality contents into the final output.
    
    \item
    There may be instances where a collective of advertisers wishes to propose an output. In such cases, the LLM may advertise multiple companies within the output, generating revenue from a subset of them. In this scenario, all collaborative efforts must be managed by the advertisers, potentially making the process less scalable and more challenging to implement.
\end{itemize}

We observe that because of the aforementioned issues, conducting LLM advertising when advertisers are tasked with altering outputs might not be a viable option. Conversely, if the AI chat-bot retains the responsibility for generating modified outputs, a different set of challenges will come into play:

\begin{itemize}
    \item advertisers need to evaluate modified outputs, in fact, as the new output is generated on the other side, advertiser needs to ensure whether it satisfies the requirements or not.
    This makes the process a bit difficult as the advertisers needs to evaluate the text and then bid on that.
    \item As a result of the previous point, the process of generating new outputs and bidding will become separated.
\end{itemize}

Above challenges seem more doable, thus, we focus on this setting in this paper.

\paragraph{How to run the auction?} 


==> related.tex <==

\begin{figure*}
    \begin{center}
    \includegraphics[width=\linewidth]{figures/personalized-ad.pdf}
    \end{center}
    \vspace{-2mm}
    \caption{An example of ChatGPT 4 providing different output tailored to the user context. We keep the context provided in Figure~\ref{fig:intro}, but asks again to advertise again to the specified user segment.}
    \label{fig:personalized-ad}
\end{figure*}

\section{Related works}
 % \krcomment{i'll add some stuff later.}
Here we present related works on LLM, online advertisement system, and their intersection.
Further related works can be found in Appendix~\ref{apd:further-rel}.

% The intersection of artificial intelligence, natural language processing, and conversational agents has witnessed significant advancements in recent years.
% The advent of the Transformer architecture, introduced in \cite{vaswani2017attention}, laid the foundation for large language models.
% Transformers, with their self-attention mechanism, revolutionized the way models capture contextual information, enabling superior performance on NLP tasks.
% By scaling up those architectures, OpenAI's GPT-3 \citep{brown2020language} and Google's BERT \citep{devlin2019bert} are obtained, revolutionizing the field of chatbots, enabling more natural and contextually relevant interactions. 
% Those models showed remarkable performance on the natural language generation task leading to the development of chatbots and conversational AI systems.
% These chatbots engage in context-aware, human-like conversations, offering valuable solutions in customer service, healthcare, and educational domains \cite{abd2020effectiveness, nicolescu2022human}.

\paragraph{Large Language Models}
Advancements in AI, NLP, and conversational agents, driven by Transformer architecture \citep{vaswani2017attention},
have given rise to models like GPT-3 \citep{brown2020language} and BERT \citep{devlin2019bert}.
These models revolutionize chatbots, enabling context-aware, human-like interactions across diverse domains \citep{abd2020effectiveness, nicolescu2022human}.
Everyday use of language models has led researchers to investigate the content generated by these models to ensure that they do not hallucinate \citep{guerreiro2023hallucinations, Ji_2023, li2023halueval, zhang2023siren} in their outputs, and do not generate harmful or biased content \citep{pmlr-v139-liang21a, navigli2023biases, NEURIPS2021_1531beb7, shen2023large, weidinger2021ethical, liu2023aligning}. In fact, trustworthy of LLMs is actively studying by researchers \citep{liu2024trustworthy}.

% \sscomment{Keivan: Discuss briefly about LLM alignment as we will discuss hallucination sort of things in DCO part.} \krcomment{is that fine?}


\paragraph{Online Advertisement}
Online advertising, particularly within the context of sponsored search auctions, has evolved in recent years,
with notable contributions from prior research.
Sponsored search auctions have been a subject of extensive investigation, emphasizing the optimization of bidding strategies and keyword relevance.\footnote{Online advertisement can be categorized by either of search or display ads. We here focus on search ads.}
\citet{edelman2007internet} provided valuable insights into the economics of sponsored search auctions,
shedding light on the intricate dynamics of keyword auctions.
\citet{goel2009contract} proposed a contract auction between the advertiser and the publisher, and introduce impression-plus-click pricing for sponsored search auction as an application. We refer to the book by \citet{roughgarden2010algorithmic} for more detailed discussion.
% \slcomment{This citation is a book chapter, not an entire book.}

% \sscomment{Cite Contract Auctions for Sponsored Search}

\paragraph{Mechanism design with LLM agents}
\citet{duetting2023mechanism} recently proposes a mechanism design problem when the bidders are LLM agents.
More specifically, the bidders bid on desired distributions of the \emph{next token}, given the history of the tokens.
They denote this problem by \emph{token auction}, and provide theoretical foundations of what a reasonable mechanism should look like.
Indeed, their model can be considered as a version of our advertiser modification and dynamic bidding framework.
Notably, they require the advertisers to provide their desired distribution and corresponding bidding for every token, which may require significant communication burden to run the mechanism in practice.
In contrast, the advertisers in our framework only bid once for the modified output, thereby inducing less communication cost.\footnote{In Section~\ref{sec:discuss-auction} and Appendix~\ref{apd:further-discuss}, we provide further discussion on~\cite{duetting2023mechanism} to compare it with our framework and how one can practically adapt their mechanism design perspective in online advertisement system within our framework.}

% \paragraph{Auctions for LLM Summary}
% A recent work by 


\paragraph{Chatbot advertisement}
% \sscomment{Skip this or move to the appendix}
With emergence of chat-bot in various websites,  several companies started to run a chat-bot advertisement, which is often referred to as sponsored message.
In the chat-bot advertisement, the companies send some private messages on the chat-bot conversation to advertise some products.
This is very different from operating an~online advertisement system over LLM, since chat-bot advertisement simply sends some messages, but our model captures the scenario in which the user asks a query and then LLM provides a output including some advertisements.
Notably, Microsoft Bing started to operate an online advertisement with Bing chat-bot (\eg see articles ~\cite{Adweek, Techcrunch, Microsoft}).
Indeed, once the user inputs a query in the chat-bot, the output often includes advertisements with explicit flags that indicates this is an advertisement.

\paragraph{Dynamic creative optimization}
Dynamic Creative Optimization (DCO) is an online advertising strategy that involves dynamically tailoring the content of an ad based on user behavior, demographics, and user context~\cite{baardman2021dynamic}. 
Instead of displaying a static, one-size-fits-all ad, DCO allows advertisers to create and serve personalized and relevant ad content to different audience segments.
By doing so the platform can improve the likelihood of user engagement, click throughs, and conversions.
DCO typically involves the use of technology and algorithms to automate the process of selecting and assembling ad elements, such as images, copy, and calls-to-action, in real-time. This customization is done based on user data, collected either in real-time or from previous interactions. 
Unlike DCO has been typically used only in display advertising not search advertising~\cite{choi2020online} since the tailored ad creatives, \eg personalized hyperlinks to websites, would not have much impact for structured output of standard search engines.
Due to the unstructured nature of LLM advertisement, the use of techniques similar to dynamic creative optimization would be highly likely to be present in future.
Our paper suggests the use of LLM, more generally generative AI, to personalize the advertisement itself  to improve the relevance and quality of the advertisement.

\ssedit{
Finally, beyond using LLM for DCO, one may use it to implement a system that can help the advertisers generating the ads itself.
Indeed, there already exists a tons of online platforms such as Japser AI for copywriting, Lexica Art for blog thumbnails, and Attentive for mobile messaging, to help marketers construct their static ads.
Further, the multi-modal capability of the very recent ChatGPT-4o by OpenAI opens the possibility of supporting advertisers creating ad assets with text-based interactions.
In addition, Meta recently introduced an AI sandbox in their~\cite{MetaAdvantage} that can help advertisers from several perspectives, including creating a variant of the given ad, constructing an ad based on text prompts or quickly changing the ad format with respect to specified ad channels~\citep{MetaSandbox}.
}


% \ssedit{
%     Recently, 
% }
% \sscomment{Discuss recent Google paper as well}

% To the extent of our knowledge, however, this is the first paper to discuss technical challenges and feasible architectures in leveraging online advertisement system with LLM.


% Recently, several tech companies started to run Chatbot advertisements.


% \begin{enumerate}
%     \item Chatbot advertising effectiveness: When does the message get through?. This paper is about Facebook sending "sponsored message" to the user, which is very different from what we are doing. This is basically referred to as Chatbot Marketing
% \end{enumerate}
% Several reference links that consider similar questions here, mostly by Microsoft Bing.
% \begin{enumerate}
%     \item \href{https://www.adweek.com/media/microsoft-details-how-advertising-works-on-bings-ai-driven-chat-based-search/}{article 1}
%     \item \href{https://about.ads.microsoft.com/en-us/blog/post/may-2023/a-new-solution-to-monetize-ai-powered-chat-experiences}{article 2}
%     \item \href{https://techcrunch.com/2023/03/29/that-was-fast-microsoft-slips-ads-into-ai-powered-bing-chat/}{article 3}
%     \item \href{https://www.thedrum.com/news/2023/03/30/gpt-4-powered-bing-chat-introduces-ads-and-experts-believe-it-s-natural-fit}{article 4}
% \end{enumerate}



==> requirements.tex <==
\section{Requirements}\label{sec:require}
In this section, we outline our expectations for LLMA, which should be evaluated based on the following criteria:

% \begin{itemize}
%     \item \textbf{Privacy}:
%     In any advertisement system where users and advertisers interact, it is imperative to maintain the confidentiality of users' privacy.
%     In essence, all aspects pertaining to a user's context, information, and data must be kept secure, as any inadvertent disclosure can pose significant risks.
    
%     \item \textbf{Reliability}: LLM advertisement systems need to associate with advertisers, making the entire system vulnerable to any kind of harmful behavior from advertisers.
%     In order to mitigate that, LLM providers should closely consider all aspects of the interaction, ensuring the reliability of the system.

%     \item \textbf{Latency}:
%     Users expect rapid interaction with LLM service, e.g., ChatGPT typically generates prompt responses, without any noticeable delay.
%     Incorporating advertisement in LLM output, inevitably, will add some latency to the overall system.
%     Nevertheless, this added delay should be minimal, ensuring that it does not significantly disrupt the user experience.

%     \item \textbf{User's satisfaction}:
%     When an advertisement is added to LLM output, it's crucial to maintain a high level of quality in the generated content.
%     Users do not wish to encounter an excessive amount of advertising in the generated responses,
%     especially when it doesn't align with their search or interests.
%     In fact, the quality of generated output should remain high, effectively addressing users' questions, concerns, etc. 
%     Advertisement involvement should not significantly degrade LLM output, as doing so would lead to reduced user satisfaction.
    
%     \item \textbf{Advertisers' satisfaction}:
%     As advertisers pay LLM providers to involve advertisements in LLM output, they expect appropriate exposure of ads in those outputs.
%     Whether it's products, services, or any other form of advertising, they expect these items to be showcased in a compelling and engaging manner within the output
%     This presentation should be interesting for users, ultimately driving revenue for the advertisers.
    
%     \item \textbf{LLM provider revenue}: 
%     Obtaining revenue is the primary goal of providing LLM advertisement services, thus,
%     LLM providers should ensure that the total additional cost of advertisement is compensated by the revenue obtained from advertisers.
%     it is worth noting that advertisements may potentially reduce the overall number of users engaging with the system, which could have adverse effects on LLM providers.
% \end{itemize}

\subsection{System requirement}

% \begin{enumerate}
%     \item (Privacy) In any advertisement system where users and advertisers interact, it is imperative to maintain the confidentiality of users' privacy.
%     In essence, all aspects pertaining to a user's context, information, and data must be kept secure, as any inadvertent disclosure can pose significant risks.
%     \item (Reliability) LLMA needs to associate with advertisers, making the entire system vulnerable to harmful behaviors from them.
%     To mitigate that, LLMA should consider every possible aspect of the behavior of the advertisers,
%     ensuring the reliability and alignment of the system~\citep{hendrycks2020aligning}.
%     \item (Latency) Users expect rapid interaction with LLM service, e.g., ChatGPT typically generates prompt responses, without any noticeable delay.
%     Incorporating advertisement in LLM output, inevitably, will add some latency to the overall system.
%     Nevertheless, this added delay should be minimal, ensuring that it does not significantly disrupt the user experience.
% \end{enumerate}

\paragraph{Privacy}
In any advertisement system where users and advertisers interact, it is imperative to maintain the confidentiality of users' privacy.
In essence, all aspects pertaining to a user's context, information, and data must be kept secure, as any inadvertent disclosure can pose significant risks.

\paragraph{Reliability} 
LLMA needs to associate with advertisers, making the entire system vulnerable to harmful behaviors from them.
To mitigate that, LLMA should consider every possible aspect of the behavior of the advertisers,
ensuring the reliability and alignment of the system~\citep{hendrycks2020aligning}.
% \slcomment{This sounds related to the concept of ``alignment'' and we may want to cite work in that area. It's also associated with the goal of influencing LLM output, as far as I understand.}

\paragraph{Latency}
Users expect rapid interaction with LLM service, e.g., ChatGPT typically generates prompt responses, without any noticeable delay.
Incorporating advertisement in LLM output, inevitably, will add some latency to the overall system.
Nevertheless, this added delay should be minimal, ensuring that it does not significantly disrupt the user experience.

\subsection{Player incentive}
\paragraph{User satisfaction}
When an advertisement is added to LLM output, it's crucial to maintain a~high level of quality in the generated content.
Users do not wish to encounter an excessive amount of advertising in the generated responses,
especially when it doesn't align with their search or interests.
% In fact, the quality of generated output should remain high, effectively addressing users' questions, concerns, etc. 
Advertisement involvement should not significantly degrade LLM output, as doing so would lead to reduced user satisfaction, thereby decreasing the user retention.
For instance, in modern online advertisement system, this is often handled using floor prices to filter out irrelevant ads to maintain the quality of the user experience. 
Similarly for LLM service, we need to ensure the final modified output including advertisements can still be a high-quality response to the user, not deviating significantly from what LLM originally would generate.
% \sscomment{Mention this one for LAS as well} \krcomment{Added, please double check Suho.}
% \slcomment{In online ads this is often handled using floor prices, i.e., the floor prices are used to filter out irrelevant ads (unless their bids are really high for some reason, like remarketing), not to directly maximize revenue.}

\paragraph{Advertisers satisfaction}
As advertisers pay LLMA to include advertisements in their outputs,
they expect appropriate exposure of ads in them.
Whether their products, services, or any other form of advertising, they expect these items to be showcased in a compelling and engaging manner within the output.
This presentation should be interesting for users, ultimately driving revenue for the advertisers.

\paragraph{Platform revenue}
Obtaining revenue is the primary goal of operating LLMA, thus,
LLMA should ensure that the total additional cost of advertisement is compensated by the revenue obtained from advertisers.
It is worth noting that advertisements may potentially reduce the overall number of users engaging with the system, which could have adverse effects on LLM itself.


% In the next section, we provide several architectures for LLM advertisement and evaluate them in terms of the above criteria.


